Fermion mass hierarchies from vector-like families and possible explanations for the electron and muon anomalous magnetic moments

This thesis covers a few successes of the SM and its limitations. The limitations implement that the SM must be expanded to explain the observables which can not be addressed by the SM such as mass of neutrinos, a few of anomalies, DM, DE, etc. In order to extend the SM, we take the model-dependent approach and a minimal extension to the SM. For the minimal extension, we make use of vector-like family, SM-like scalar (plus a singlet flavon), and $U(1)^\prime$ symmetry. A first BSM model in my first work is to explain both the electron and muon anomalous magnetic moments at the same time, while keeping the constraints $\mu \rightarrow e \gamma$ decay and neutrino trident production. Especially, two mass sources, chirality flip and vector-like mass, appear in our analytic prediction for the anomalies and the chirality flip mass between $0$ and $200 \operatorname{GeV}$ is searched and then we show no any value between them can satisfy the anomalies at the same time. A second BSM model in my second work shares the same motivation, to explain both anomalies, however it goes one step further by considering the strong hierarchical structure of the SM into the second BSM model. In this BSM model, the SM appears as an effective theory spontaneously broken from the $U(1)^\prime$ symmetry. Both anomalies are studied in the neutrino sector first and it reveals that the neutrino contributions are too small to explain their experimental bounds, so leading to a conclusion that the neutrinos can not explain both anomalies simultaneously. Next we study the scalar contribution and show that the scalar contributions can explain both anomalies simultaneously. My third work investigate the diverse FCNCs within the same second BSM model to constrain mass range of vector-like fermions.

==> TheSecondpaper.tex <==
%% ----------------------------------------------------------------
%% TheSecondpaper.tex
%% ---------------------------------------------------------------- 
\chapter{Non-standard contributions to the muon and electron anomalous magnetic moments : $W$ gauge boson exchange} \label{Chapter:The2ndpaper}

\section{$W$ boson exchange contributions to $(g-2)_\mu, (g-2)_e$ and $\func{BR}\left( \mu \rightarrow e \gamma \right)$} \label{sec:second_paper_Wexchange}

Within the framework of our proposed model, we start by investigating the
muon and electron anomalous magnetic moments with $W$ boson exchange first. 
%For this task, the
%relevant sector is neutrinos so 
Given that such $W$ boson exchange contribution also involves virtual
neutrinos in the internal lines of the loop, we revisit the mass matrix for
neutrinos. In this mass matrix, we remove fifth vector-like neutrinos $%
\nu_{5R}$ and $\widetilde{\nu}_{5R}$ since they are too heavy to contribute
to the phenomenology under study. As mentioned in the previous section, we
stick to a condition where the coefficient $y$ is expected to be of order
unity, %in which order of the coefficient $y$ is ideally unity, 
%while that
whereas the coupling $x$ is expected to be smaller than $y$. 
%of $x$ is quite smaller than that of $y$. 
%The
Such condition can be easily seen by substituting the coefficients $%
y_{i4}^\nu$ by $y_{i}^\nu$ and the coefficients $x_{i4}^L$ by $\epsilon
y_{i}^{\nu \prime}$ where $\epsilon$ is a suppression factor. Putting all
these considerations together, the mass matrix for neutrinos in Equation \ref%
{eqn:mass_matrix_neutrinos} after electroweak symmetry breaking takes the
form:%is reduced to:
\begin{equation}
M^\nu \approx \left( 
\begin{array}{c|ccc|cc}
& \nu_{1L} & \nu_{2L} & \nu_{3L} & \overline{\nu}_{4R} & \widetilde{\nu}_{4R}
\\ \hline
\nu_{1L} & 0 & 0 & 0 & y_{1}^\nu v_u & \epsilon y_{1}^{\nu \prime} v_d \\ 
\nu_{2L} & 0 & 0 & 0 & y_{2}^\nu v_u & \epsilon y_{2}^{\nu \prime} v_d \\ 
\nu_{3L} & 0 & 0 & 0 & y_{3}^\nu v_u & \epsilon y_{3}^{\nu \prime} v_d \\ 
\hline
\overline{\nu}_{4R} & y_{1}^\nu v_u & y_{2}^\nu v_u & y_{3}^\nu v_u & 0 & 
M_{44}^{\nu} \\ 
\widetilde{\nu}_{4R} & \epsilon y_{1}^{\nu \prime} v_d & \epsilon y_{2}^{\nu
\prime} v_d & \epsilon y_{3}^{\nu \prime} v_d & M_{44}^{\nu} & 0%
\end{array}
\right) \equiv \left( 
\begin{array}{cc}
0 & m_D \\ 
m_D^T & M_N%
\end{array}
\right) , \label{eqn:mass_matrix_neutrinos_reduced}
\end{equation}
where $v_u(v_d)$ is the vev of $\widetilde{H}_u(H_d)$, $v_u$ runs from $246/%
\sqrt{2}\func{GeV} \simeq 174 \func{GeV}$ to $246 \func{GeV}$ and $%
v_u^2+v_d^2 = \left( 246 \func{GeV} \right)^2$.

\subsection{Type 1b seesaw mechanism} \label{sec:second_paper_type1b_seesaw}

Now that we constructed the neutrino mass matrix for this task, the next
step is to read off the operator which gives rise to the neutrino mass from
the mass matrix. Generally, the well-known operator for neutrino mass is the
Weinberg operator(type 1a seesaw mechanism) $\frac{1}{\Lambda}L_i L_j H H$.
A main feature of the Weinberg operator is the same SM Higgs should be repeated
in the operator, however that %process 
property is not present in our model %does not work in this model
since the Higgs doublets $H_{u,d}$ are negatively charged under the $%
U(1)^{\prime}$ symmetry, which implies %and  it necessarily leads to
the corresponding Weinberg operator having such fields will not be invariant
under the $U(1)^{\prime}$ unless an insertion of a quadratic power of the
gauge singlet scalar $\phi$ is considered. However we do not consider the
operators $\frac{1}{\Lambda^3}(\bar{L}_i\tilde{H}_u)(\tilde{H}%
_uL^C_j)(\phi^*)^2$ and $\frac{1}{\Lambda^3}(\bar{L}_iH_d)(H_dL^C_j)\phi^2$
in the neutrino sector, since they are very subleading and thus will give a
tiny contribution to the light active neutrino masses. 
%will provide a very sul violation of quantum number. 
Instead of relying on a seven dimensional Weinberg to generate the tiny
masses for the light active neutrinos, we take another approach named type
1b seesaw mechanism (we call the Weinberg operator ``type 1a seesaw
mechanism" to differentiate with) %in which
where the mixing of different $SU(2)$ Higgs doublets can appear satisfying
charge conservation. Diagrams for the operators are given in Figure \ref%
{fig:diagrams_type1ab_operators} for comparison:
\begin{figure}[]
\centering
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{Comp_1a_1b_1}
\end{subfigure} \hspace{0.1cm} 
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{Comp_1a_1b_2}
\end{subfigure}
\caption{Diagrams which lead to effective Weinberg operators for the
Majorana and vector-like mass in the mass insertion approximation, where $%
i,j=1,2,3$ and $k=4$, respectively. The left is the Weinberg operator(or
type 1a seesaw mechanism) in which mass $M$ is Majorana mass and the right
is Weinberg-like operator(or type 1b seesaw mechanism) in which mass $M$ is
vector-like mass.}
\label{fig:diagrams_type1ab_operators}
\end{figure}
The diagrams in Figure \ref{fig:diagrams_type1ab_operators} clearly tell the
difference between Majorana mass and vector-like mass. They share a common
property that they violate the lepton number conservation, %while
whereas the particles appearing in %for 
a Majorana mass term are same but those ones involved in vector-like mass
terms are different. As the type 1b seesaw mechanism only works in this
model, we make use of this seesaw mechanism for the analysis of neutrinos.
With the operator, the renormalizable Lagrangian for neutrinos can be
written as:
\begin{equation}
\begin{split}
\mathcal{L}_{\nu}^{\func{Yukawa+Mass}} = y_{i}^{\nu} \overline{L}_{iL} 
\widetilde{H}_u \nu_{kR} + \epsilon y_i^{\nu\prime} \overline{L}_{iL} H_d 
\overline{\widetilde{\nu}}_{kR} + M_{kk}^{M} \overline{\widetilde{\nu}}_{kR}
\nu_{kR} + \func{h.c.} , \label{eqn:Lagrangian_neutrinos}
\end{split}%
\end{equation}
where $i = 1,2,3$ and $k=4$. The renormalizable Lagrangian of Equation %
\ref{eqn:Lagrangian_neutrinos} above the electroweak scale %is down to an
generates an effective Lagrangian after decoupling the heavy vector-like
neutrinos, which is suitable for study of low energy neutrino phenomenology.
The effective Lagrangian for neutrino at electroweak scale is given by\cite%
{Hernandez-Garcia:2019uof}
\begin{equation}
\mathcal{L}^{d=5} = c_{ij}^{d=5} \left( \left( L_i^T \widetilde{H}_u \right)
\left( H_d^T L_j \right) + \left( L_i^T H_d \right) \left( \widetilde{H}_u^T
L_j \right) \right),  \label{eqn:effective_operators_neutrinos}
\end{equation}
where the coefficient $c_{ij}^{d=5}$ is suppressed by a factor of the
vector-like mass $M$. The neutrino mass matrix of Equation \ref%
{eqn:mass_matrix_neutrinos_reduced} can be diagonalized by the unitary
matrix $U$ as below:
\begin{equation}
U^T 
\begin{pmatrix}
0 & m_D^T \\ 
m_D & M_N%
\end{pmatrix}
U = 
\begin{pmatrix}
m_\nu^{\func{diag}} & 0 \\ 
0 & M_N^{\func{diag}}%
\end{pmatrix},
\label{eqn:diagonalization_neutrinos}
\end{equation}
where $m_\nu^{\func{diag}}$ is a diagonal matrix for the light left-handed
neutrinos $\nu_{iL}$ and $M_N^{\func{diag}}$ is that for the heavy
vector-like neutrinos $\nu_{4R}, \widetilde{\nu}_{4R}$. Here, the unitary
mixing matrix $U$ is defined by multiplication of two unitary matrices which
we call $U_A$ and $U_B$, respectively\cite{Blennow:2011vn}:
\begin{equation}
\begin{split}
U &= U_A \cdot U_B \\
U_A &= \func{exp}%
\begin{pmatrix}
0 & \Theta \\ 
-\Theta^\dagger & 0%
\end{pmatrix}
\simeq 
\begin{pmatrix}
I-\frac{\Theta \Theta^\dagger}{2} & \Theta \\ 
-\Theta^\dagger & I-\frac{\Theta \Theta^\dagger}{2}%
\end{pmatrix}
\quad \text{at leading order in $\Theta$} \\
U_B &= 
\begin{pmatrix}
U_{\func{PMNS}} & 0 \\ 
0 & I%
\end{pmatrix}%
\end{split}
\label{eqn:unitary_matrix_neutrinos}
\end{equation}
The unitary matrix $U_{\func{PMNS}}$ in $U_B$ is the well-known
Pontecorvo-Maki-Nakagawa-Sakata matrix and is parameterized by \cite%
{Hernandez-Garcia:2019uof,Chau:1984fp}
\begin{equation}
\begin{split}
U_{\func{PMNS}} = 
&\begin{pmatrix}
1 & 0 & 0 \\ 
0 & \cos\theta_{23} & \sin\theta_{23} \\ 
0 & -\sin\theta_{23} & \cos\theta_{23}%
\end{pmatrix}
\begin{pmatrix}
\cos\theta_{13} & 0 & \sin\theta_{13} e^{-i\delta_{\func{CP}}} \\ 
0 & 1 & 0 \\ 
-\sin\theta_{13} e^{i\delta_{\func{CP}}} & 0 & \cos\theta_{13}%
\end{pmatrix} \\
& 
\begin{pmatrix}
\cos\theta_{12} & \sin\theta_{12} & 0 \\ 
-\sin\theta_{12} & \cos\theta_{12} & 0 \\ 
0 & 0 & 1%
\end{pmatrix}
\begin{pmatrix}
e^{-i\alpha^\prime/2} & 0 & 0 \\ 
0 & e^{-i\alpha/2} & 0 \\ 
0 & 0 & 1%
\end{pmatrix}%
\end{split}
,  \label{eqn:PMNS_mixing_matrix}
\end{equation}
where the Majorana phase $\alpha^\prime$ is set to zero in this model. The mixing matrices $%
U_{A,B}$ are unitary, however the $3\times 3$ upper block of the unitary
matrix $U$ is not unitary due to the %multiplied 
factor $\left( I - \Theta \Theta^\dagger/2 \right)$ for the light neutrinos. An
interesting feature of the unitary matrix $U$ is it is unitary globally, but
non-unitary locally and this non-unitarity contributes to explain muon and
electron anomalous magnetic moments. Replacing the unitary matrices in
Equation \ref{eqn:unitary_matrix_neutrinos} back to Equation \ref%
{eqn:diagonalization_neutrinos}, the result is simplified with the
assumption $M_N \gg m_D$ to the conventional seesaw mechanism:
\begin{equation}
\begin{split}
\Theta &\simeq m_D^\dagger M_N^{-1} \\
U_{\func{PMNS}}^* m_{\nu}^{\func{diag}} U_{\func{PMNS}}^\dagger &\simeq
-m_D^T M_N^{-1} m_D \equiv -m \\
M_N^{\func{diag}} &\simeq M_N,  \label{eqn:parameterisation_neutrinos}
\end{split}%
\end{equation}
where $m$ is the effective mass matrix resulted from Equation \ref%
{eqn:mass_matrix_neutrinos_reduced}.
\begin{equation}
m_{ij} = \frac{\epsilon v_u v_d}{M_{44}^{\nu}} \left( y_i^\nu
y_j^{\nu\prime} + y_i^{\nu\prime} y_j^\nu \right)
\label{eqn:effective_neutrino_mass_matrix}
\end{equation}
Therefore, smallness of the light neutrino masses can be understood not only
from mass of vector-like mass $M_{44}^{\nu}$ but also from the suppression
factor $\epsilon$ and the presence of $\epsilon$ allows more flexibility in the allowed mass values of the vector-like neutrinos. Revisiting non-unitarity part for the light neutrinos from
the unitary matrix $U$\cite{Blennow:2011vn,FernandezMartinez:2007ms}, it
reads:
\begin{equation}
\begin{split}
&\left( I - \frac{\Theta_i \Theta_j^\dagger}{2} \right) U_{\func{PMNS}} =
\left( I - \eta_{ij} \right) U_{\func{PMNS}}
\label{eqn:non_unitarity_light_neutrinos}
\end{split}%
\end{equation}
The non-unitarity $\eta$ is associated with the presence of the heavy vector-like
neutrinos and can be derived from a coefficient of the effective Lagrangian
at dimension 6\cite{Broncano:2002rw}:
\begin{equation}
\mathcal{L}^{d=6} = c_{ij}^{d=6} \left( \left( L_i^\dagger \widetilde{H}_u
\right) i\slashed{\partial} \left( \widetilde{H}_u^\dagger L_j \right) +
\left( L_i^\dagger H_d \right) i\slashed{\partial} \left( H_d^\dagger L_j
\right) \right)  \label{eqn:effective_operators_dimension6}
\end{equation}
Once the SM Higgs doublets in Equation \ref%
{eqn:effective_operators_dimension6} develop its vev, the Lagrangian at
dimension 6 causes non-diagonal kinetic terms for the light neutrinos and it
gives rise to deviations of unitarity when it is diagonalized. The
deviations of unitarity can be expressed in terms of the coefficient at
dimension 6 $\eta_{ij} \equiv v^2 c_{ij}^{d=6}/2$.
\begin{equation}
\eta_{ij} = \frac{\Theta_i \Theta_j^\dagger}{2} = \frac{1}{2} \frac{%
m_D^\dagger m_D}{M_N^2} = \frac{1}{2M_{44}^{\nu 2}} \left( v_u^2 y_i^{\nu*}
y_j^\nu + \epsilon^2 v_d^2 y_i^{\nu\prime*} y_j^{\nu\prime} \right) \simeq 
\frac{v_u^2}{2M_{44}^{\nu 2}} y_i^{\nu *} y_j^{\nu}
\label{eqn:deviation_of_unitarity}
\end{equation}
From the fourth term in Equation \ref{eqn:deviation_of_unitarity}, the term
with $\epsilon^2$ can be safely ignored due to both relative
smallness of $v_d$ and the suppression factor $\epsilon$. Thus, the
deviation of unitarity $\eta$ consists of the vector-like mass $M_{44}^{\nu}$
and the Yukawa couplings $y_{i,j}^\nu$. As an interesting example, it is
possible that the Yukawa couplings $y_{i,j}^\nu$ can be obtained from the
observables such as the PMNS mixing matrix and two mass squared splitting, $%
\Delta m_{sol}^2$ and $\Delta m_{atm}^2$, in the neutrino oscillation
experiments. Since the hierarchy between the light neutrinos is not yet
determined, there are two possible scenarios, normal hierarchy(NH) and
inverted hierarchy(IH), and the lightest neutrino remains massless, whereas two
other neutrinos get massive. The Yukawa couplings $y_{i}^{\nu,\nu\prime}$
for the NH($m_1 = 0$) are determined by
\begin{equation}
\begin{split}
y_i^\nu &= \frac{y}{\sqrt{2}} \left( \sqrt{1+\rho} \left( U_{\func{PMNS}}^*
\right)_{i3} + \sqrt{1-\rho} \left( U_{\func{PMNS}}^* \right)_{i2} \right) \\
y_i^{\nu\prime} &= \frac{y^\prime}{\sqrt{2}} \left( \sqrt{1+\rho} \left( U_{%
\func{PMNS}}^* \right)_{i3} - \sqrt{1-\rho} \left( U_{\func{PMNS}}^*
\right)_{i2} \right),
\end{split}%
\end{equation}
where $y$ and $y^\prime$ are real numbers and $\rho=(1-\sqrt{r})/(1+\sqrt{r}%
) $ with $r \equiv \lvert \Delta m_{sol}^2 \rvert/\lvert \Delta m_{atm}^2
\rvert = \Delta m_{21}^2/\Delta m_{31}^2$, whereas the Yukawa couplings $y_i^{\nu,\nu\prime}$ for the IN($m_3=0$) are
\begin{equation}
\begin{split}
y_i^\nu &= \frac{y}{\sqrt{2}} \left( \sqrt{1+\rho} \left( U_{\func{PMNS}}^*
\right)_{i2} + \sqrt{1-\rho} \left( U_{\func{PMNS}}^* \right)_{i1} \right) \\
y_i^{\nu\prime} &= \frac{y^\prime}{\sqrt{2}} \left( \sqrt{1+\rho} \left( U_{%
\func{PMNS}}^* \right)_{i2} - \sqrt{1-\rho} \left( U_{\func{PMNS}}^*
\right)_{i1} \right),
\end{split}%
\end{equation}
where $\rho=(1-\sqrt{1+r})/(1+\sqrt{1+r})$ with $r \equiv \lvert \Delta
m_{sol}^2 \rvert/\lvert \Delta m_{atm}^2 \rvert = \Delta m_{21}^2/\Delta
m_{32}^2$.

\subsection{The charged lepton flavour violation (CLFV) $\mu \rightarrow e \gamma$ decay} \label{sec:second_paper_W_mueg}

Consider the three light neutrinos in the SM for the CLFV $\mu \rightarrow e \gamma$
decay first. In this case, the unitary mixing matrix becomes just the PMNS
mixing matrix and the GIM mechanism which suppresses flavour-changing
process works, therefore it leads quite suppressed sensitivity for $\func{BR}%
\left(\mu \rightarrow e \gamma\right)$ about $10^{-55}$\cite{Calibbi:2017uvl}%
, which is impossible to observe with the current sensitivity of $\mu
\rightarrow e \gamma$ decay. This impractical sensitivity can be enhanced to
the observable level by introducing the heavy vector-like neutrinos which give
rise to deviation of unitarity. With the presence of heavy vector-like
neutrinos, the GIM mechanism is gone and the factor suppressed by GIM
mechanism can survive with a factor of deviation of unitarity, which plays a
crucial role to increase significantly order of theoretical prediction for $%
\mu \rightarrow e \gamma$ decay\cite{Glashow:1970gm}. Therefore, the
strongest constraint for deviation of unitarity in the modified PMNS mixing
matrix comes from CLFV $\mu \rightarrow e \gamma$ decay. The possible one-loop
diagrams for the CLFV $\mu \rightarrow e \gamma$ with all neutrinos in this
model are given in Figure \ref{fig:diagrams_muegamma_with_allneutrinos}.
\begin{figure}[]
\centering
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{muegamma_neutrinos_muon}
\end{subfigure} \hspace{0.1cm}
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{muegamma_neutrinos_electron}
\end{subfigure}
\caption{Diagrams for CLFV $\protect\mu \rightarrow e \protect\gamma$ decay
with all neutrinos. Here $n=1,2,3,4,5$.}
\label{fig:diagrams_muegamma_with_allneutrinos}
\end{figure}
The amplitude from above diagrams in Figure \ref%
{fig:diagrams_muegamma_with_allneutrinos} reads\cite{Calibbi:2017uvl}:
\begin{equation}
\begin{split}
\mathcal{M}\left( \mu \rightarrow e \gamma \right) &= \overline{u}_e i
\sigma_{\mu\nu} q^{\nu} \left( F_1 + F_2 \gamma^5 \right) u_\mu
\epsilon^{*\mu} \\
&= \overline{u}_e i \sigma_{\mu\nu} q^{\nu} \left( A_R P_R + A_L P_L \right)
u_\mu \epsilon^{* \mu},  \label{eqn:amplitude_muegamma_W}
\end{split}%
\end{equation}
where $u$ is Dirac spinor for the muon and electron, $q$ is
four momentum of an outgoing photon, $F_{1,2}$ are form factors, $%
A_{L,R}$ are left- and right-handed amplitude defined to be $A_{L,R} = F_1
\pm F_2$ and lastly $P_{L,R}$ are projection operators. From the amplitude,
the helicity flip between initial particle and final particle should arise
and this makes the helicity flip process takes place on one of external legs
since the $W$ gauge boson couples only to left-handed fields. Comparing the
left diagram with the right, the left is proportional to the muon mass,
while the right is proportional to the electron mass, which means that
impact of the right is ignorable. The unpolarized squared amplitude $\lvert 
\mathcal{M} \rvert^2$ takes the form:
\begin{equation}
\lvert \mathcal{M} \rvert^2 = m_\mu^4 \left( A_R + A_L \right)^2 \simeq
m_\mu^4 \left( A_R \right)^2  \label{eqn:unpolarised_squared_amplitude}
\end{equation}
Then, the decay rate is given by
\begin{equation}
\Gamma\left( \mu \rightarrow e \gamma \right) = \frac{\lvert \mathcal{M}
\rvert^2}{16\pi m_\mu} = \frac{m_\mu^3}{16\pi} \lvert A_R \rvert^2
\label{eqn:decay_rate_muegamma}
\end{equation}
where $A_R$ is expressed by\cite{Cheng:1985bj,Calibbi:2017uvl}\footnote{%
Since the PMNS mixing matrix is multiplied by a factor of deviation of
unitarity, it is not unitary any more. Therefore, the first term of sum over
neutrino eigenstates in Equation (28) of \cite{Calibbi:2017uvl} does not
vanish and come in our prediction with a loop function $F(x_n)$.}
\begin{equation}
A_R = \frac{g^2 e}{128\pi^2} \frac{m_\mu}{M_W^2} \sum_{n=1,2,3,4,5} U_{2 n}
U_{1 n}^* F(x_n) \left[ 1 - \frac{1}{3} \frac{\ln \xi}{\xi-1} + \frac{1}{%
\xi-1} \left( \frac{\xi \ln \xi}{\xi-1} - 1 \right) \right]
\label{eqn:left_handed_amplitdue_AR}
\end{equation}
Taking the unitary gauge into account, $\xi \rightarrow \infty$, the
additional $\xi$-dependent terms in $A_R$ all are cancelled by contribution
of Goldstone bosons so $A_R$ is gauge invariant. Substituting the gauge
invariant $A_R$ back into the decay rate of Equation \ref%
{eqn:decay_rate_muegamma} and dividing the expanded decay rate by the total
muon decay rate $\Gamma\left(\mu \rightarrow e \nu \overline{\nu} \right) =
G_F^2 m_\mu^5/192\pi^3$, we have the prediction for $\mu \rightarrow e
\gamma $ decay\cite{Hernandez-Garcia:2019uof,Calibbi:2017uvl}:
\begin{equation}
\func{BR}\left(\mu \rightarrow e \gamma \right) = \frac{\Gamma \left( \mu
\rightarrow e \gamma \right)}{\Gamma \left( \mu \rightarrow e \nu_\mu 
\overline{\nu}_e \right)} = \frac{3\alpha}{32\pi} \frac{\lvert \sum_{n=1}^5
U_{2n} U_{n1}^{\dagger} F(x_n) \rvert^2}{\left( U U^{\dagger} \right)_{11}
\left( U U^{\dagger} \right)_{22}} , \label{eqn:prediction_muegamma_neutrinos}
\end{equation}
where $x_n = M_n^2/M_W^2$ and the loop function $F(x_n)$ is
\begin{equation}
F(x_n) = \frac{10 - 43 x_n + 78 x_n^2 - (49 - 18 \log x_n) x_n^3 + 4 x_n^4}{%
3(x_n-1)^4}.  \label{eqn:loop_function_F}
\end{equation}
Numerator in Equation \ref{eqn:prediction_muegamma_neutrinos} can be
simplified by separating the light neutrinos and heavy vector-like neutrinos as
below(Contribution of the fifth neutrino $\widetilde{\nu}_{4R}$ is safely ignored both by the
suppression factor $\epsilon$ and by relative smallness of $v_d$ compared to 
$v_u$):
\begin{equation}
\begin{split}
\lvert \sum_{n=1}^5 U_{2n} U_{n1}^{\dagger} F(x_n) \rvert^2 &\simeq \lvert
U_{2i} U_{i1}^\dagger F(0) + U_{24} U_{41}^\dagger F(x_4) \rvert^2 \\
U_{2i} U_{i1}^{\dagger} &= -\eta_{12}^* - \eta_{21} = -2\eta_{21} \\
U_{24} U_{41}^{\dagger} &= \Theta_{24} \Theta_{14}^* = 2\eta_{21} \\
\lvert \sum_{n=1}^5 U_{2n} U_{n1}^{\dagger} F(x_n) \rvert^2 &\simeq \lvert
4\eta_{21} \rvert^2 \left( F(x_4) - F(x_0) \right)^2
\label{eqn:numerator_simplified}
\end{split}%
\end{equation}
The final form for the CLFV $\mu \rightarrow e \gamma$ decay in this model reads:
\begin{equation}
\func{BR}\left(\mu \rightarrow e \gamma \right) = \frac{3\alpha_{\func{em}}}{%
8\pi} \lvert \eta_{21} \rvert^2 \left( F(x_4) - F(0) \right)^2,
\label{eqn:prediction_muegamma_final}
\end{equation}
where $\alpha_{\func{em}}$ is the fine structure constant. We find that our
theoretical prediction for the $\mu \rightarrow e \gamma$ decay can be expressed
in terms of the deviation of unitarity $\eta_{21}$.

\subsection{The anomalous muon magnetic moment $g-2$} \label{sec:second_paper_W_mug2}

We derive our prediction for the muon anomalous magnetic moment in this
section and confirm the derived expression can be consistent with an
expression of the theoretical prediction for $\mu \rightarrow e \gamma$ in
references\cite{Calibbi:2017uvl,Lindner:2016bgg}. Consider two possible
diagrams for muon anomalous magnetic moment at one-loop level in Figure \ref%
{fig:diagrams_muong2_with_allneutrinos}.
\begin{figure}[H]
\centering
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{muong2_neutrinos_1}
\end{subfigure} \hspace{0.1cm}
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{muong2_neutrinos_2}
\end{subfigure}
\caption{Diagrams for muon anomalous magnetic moment with all neutrinos. Here $n=1,2,3,4,5$.}
\label{fig:diagrams_muong2_with_allneutrinos}
\end{figure}
The amplitude for the muon anomalous magnetic moment at one-loop level is:
\begin{equation}
\begin{split}
\mathcal{M}\left( \Delta a_\mu \right) &= \overline{u}_\mu i \sigma_{\mu\nu}
q^{\nu} \left( F_1 + F_2 \gamma^5 \right) u_\mu \epsilon^{*\mu} \\
&= \overline{u}_\mu i \sigma_{\mu\nu} q^{\nu} \left( A_R P_R + A_L P_L
\right) u_\mu \epsilon^{* \mu}  \label{eqn:amplitude_muong2_W}
\end{split}%
\end{equation}
Unlike the CLFV $\mu \rightarrow e \gamma$ decay, muon anomaly diagrams have
the same structure for helicity flip process. So we conclude $A_R$ is equal
to $A_L$ and can make use of other expression of this amplitude to derive
our own expression for $\Delta a_\mu$\cite{Lindner:2016bgg}.
\begin{equation}
\begin{split}
V &= \overline{u}_\mu i \sigma_{\alpha\beta} q^\beta e m_\mu \left(
A_{\mu\mu}^M + \gamma_5 A_{\mu\mu}^E \right) u_\mu \epsilon^{*\alpha} \\
&= \overline{u}_\mu i \sigma_{\alpha \beta} q^{\beta} e m_\mu \left( \left(
A_{\mu\mu}^M + A_{\mu\mu}^E \right) P_R + \left( A_{\mu\mu}^M - A_{\mu\mu}^E
\right) P_L \right) u_\mu \epsilon^{*\alpha}
\end{split}
\label{eqn:amplitude_muong2_W_LiviewonLFV}
\end{equation}
Comparing Equation \ref{eqn:amplitude_muong2_W} with Equation \ref%
{eqn:amplitude_muong2_W_LiviewonLFV}, we confirm that
\begin{equation}
\begin{split}
A_R &= e m_\mu \left( A_{\mu\mu}^M + A_{\mu\mu}^E \right) \\
A_L &= e m_\mu \left( A_{\mu\mu}^M - A_{\mu\mu}^E \right)
\label{eqn:equality_ALR_AME}
\end{split}%
\end{equation}
Here, we can use the condition that $A_R = A_L$ identified in Figure \ref%
{fig:diagrams_muong2_with_allneutrinos} and can rearrange $A_{L,R}$ in terms
of $A_{\mu\mu}^{M,E}$, which are essential to derive our theoretical muon
anomaly prediction. Then, we find our desirable form $A_{\mu\mu}^{M,E}$ for
the muon anomalous magnetic moment.
\begin{equation}
\begin{split}
A_{\mu\mu}^M &= \frac{1}{e m_\mu} A_R = \frac{g^2}{128\pi^2} \frac{1}{M_W^2}
\sum_{n=1,2,3,4,5} U_{2n} U_{2n}^* F(x_n) \\
A_{\mu\mu}^E &= 0  \label{eqn:redefinition_AME}
\end{split}%
\end{equation}
Using the definition for both the muon anomalous magnetic moment and branching
ratio of $\mu \rightarrow e \gamma$ decay in \cite{Lindner:2016bgg}, we can
check our analytic argument for the observable and constraint are correct.
\begin{equation}
\begin{split}
\Delta a_\mu &= A_{\mu\mu}^M m_\mu^2 \\
\func{BR}\left( \mu \rightarrow e \gamma \right) &= \frac{3(4\pi)^3 \alpha_{%
\func{em}}}{4G_F^2} \left( \lvert A_{\mu e}^M \rvert^2 + \lvert A_{\mu e}^E
\rvert^2 \right)  \label{eqn:definition_muong2_muegamma_reivewonLFV}
\end{split}%
\end{equation}
One difference between $A_{\mu\mu}^{M,E}$ and $A_{L,R}$ is $%
that A_{\mu\mu}^{M,E} $ is only determined by the internal structure of the loop in
Figure \ref{fig:diagrams_muong2_with_allneutrinos}, whereas $A_{L,R}$ is the
extended factor by multiplying $A_{\mu\mu}^{M,E}$ by the helicity flip mass
in one of the external legs. Therefore, it is natural to think $A_{\mu\mu}^{M,E}$
is the same as $A_{\mu e}^{M,E}$ since their internal structure of loop are
exactly same\footnote{%
One can concern the coefficient at the vertex with electron. However, this
change is already reflected on the loop integration $A_R$ of Equation \ref%
{eqn:left_handed_amplitdue_AR} by $U_{1n}$. For the muon anomaly, the
coefficient is simply replaced by $U_{2n}$, therefore, modification of the
coefficient at the vertex does not harm our argument.}. The muon anomalous
magnetic moment and the branching ratio of $\mu \rightarrow e \gamma$ take
the form:
\begin{equation}
\begin{split}
\Delta a_\mu &= \frac{\alpha_W}{32\pi} \frac{m_\mu^2}{M_W^2}
\sum_{n=1,2,3,4,5} U_{2n} U_{2n}^* F(x_n) \\
\func{BR}\left(\mu \rightarrow e \gamma \right) &= \frac{3\alpha_{\func{em}}%
}{32\pi} \lvert \sum_{n=1,2,3,4,5} U_{2n} U_{1n}^* F(x_n) \rvert^2
\label{eqn:muong2_muegamma_W_ourprediction}
\end{split}%
\end{equation}
where the $\alpha_W$ is the weak coupling constant. As for the branching
ratio of $\mu \rightarrow e \gamma$ in Equation \ref%
{eqn:muong2_muegamma_W_ourprediction}, we showed that substituting $A_{\mu
e} $ back into the branching ratio in Equation \ref%
{eqn:definition_muong2_muegamma_reivewonLFV} is exactly consistent with the
one in Equation \ref{eqn:prediction_muegamma_neutrinos}. Expanding the unitary
mixing matrices in the muon anomaly prediction in Equation \ref%
{eqn:muong2_muegamma_W_ourprediction}, yields the following relation:
\begin{equation}
\Delta a_\mu = \frac{\alpha_W}{32\pi} \frac{m_\mu^2}{M_W^2} \left( (1 -
2\eta_{22})F(0) + 2\eta_{22}F(x_4) \right).
\label{eqn:expansion_muong2_ourprediction}
\end{equation}
Looking at Equation \ref%
{eqn:expansion_muong2_ourprediction}, it is clear that the SM part which is without $\eta$
and the BSM having $\eta$ are entangled together. We arrive at the right
prediction for the muon anomaly at one-loop by removing the SM part from
Equation \ref{eqn:expansion_muong2_ourprediction}
\begin{equation}
\Delta a_\mu = \frac{\alpha_W}{16\pi} \frac{m_\mu^2}{M_W^2} \eta_{22} \left(
F(x_4) - F(0) \right).  \label{eqn:expansion_muong2_correct_prediction}
\end{equation}
Similarly to the branching ratio of $\mu \rightarrow e \gamma$ decay, it can
be confirmed that the prediction for the muon anomaly also consists of the
factor of deviation of unitarity $\eta$.

\subsection{The anomalous electron magnetic moment $g-2$} \label{sec:second_paper_W_eg2}

As in the muon anomalous magnetic moment, the same diagrams with external
particles replaced by electrons can be generated in Figure \ref{fig:diagrams_electrong2_with_allneutrinos}.
\begin{figure}[H]
\centering
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{electrong2_neutrinos_1}
\end{subfigure} \hspace{0.1cm}
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{electrong2_neutrinos_2}
\end{subfigure}
\caption{Diagrams for electron anomalous magnetic moment with all neutrinos. Here $n=1,2,3,4,5$.}
\label{fig:diagrams_electrong2_with_allneutrinos}
\end{figure}
Using the complete form of the muon anomaly prediction in Equation \ref%
{eqn:expansion_muong2_correct_prediction}, we can derive the right
prediction for the electron anomalous magnetic moment with slight modifications $%
m_\mu \rightarrow m_e, \eta_{22} \rightarrow \eta_{11}$.

\begin{equation}
\Delta a_e = \frac{\alpha_W}{16\pi} \frac{m_e^2}{M_W^2} \eta_{11} \left(
F(x_4) - F(0) \right).  \label{eqn:expansion_electrong2_correct_prediction}
\end{equation}

\subsection{Numerical analysis of $W$ exchange contributions} \label{sec:second_paper_W_numeric}

The presence of heavy vector-like neutrinos leads to the deviation of
unitarity and the observables $\Delta a_{\mu,e}$ and constraint $\func{BR}%
\left(\mu \rightarrow e \gamma\right)$ can be written in terms of the factor
of non-unitarity $\eta$.
\begin{equation}
\begin{split}
\func{BR}\left(\mu \rightarrow e \gamma \right) &= \frac{3\alpha_{\func{em}}%
}{8\pi} \lvert \eta_{21} \rvert^2 \left( F(x_4) - F(0) \right)^2 \\
\Delta a_\mu &= \frac{\alpha_W}{16\pi} \frac{m_\mu^2}{M_W^2} \eta_{22}
\left( F(x_4) - F(0) \right) \\
\Delta a_e &= \frac{\alpha_W}{16\pi} \frac{m_e^2}{M_W^2} \eta_{11} \left(
F(x_4) - F(0) \right).  \label{eqn:prediction_muegamma_muong2_electrong2}
\end{split}%
\end{equation}

\subsubsection{The branching ratio of $\mu \rightarrow e \gamma$ decay}

We consider the branching ratio of $\mu \rightarrow e \gamma$ decay first.
Since we assume that mass of heavy vector-like neutrinos are heavier than $1%
\func{TeV}$, the value of $F(0)$ for the light neutrinos converges to approximately $%
3.3$, while that of $F(x_4)$ for the heavy vector-like neutrino converges to $%
1.3 $. Therefore, the branching ratio of $\mu \rightarrow e \gamma$ decay
can be reduced to\cite{Hernandez-Garcia:2019uof}
\begin{equation}
\func{BR}\left(\mu \rightarrow e \gamma \right) = \frac{3\alpha_{\func{em}}}{%
8\pi} \lvert \eta_{21} \rvert^2 \left( F(x_4) - F(0) \right)^2 \leq \frac{%
3\alpha_{\func{em}}}{2\pi} \lvert \eta_{21} \rvert^2.
\label{eqn:muegamma_simplified}
\end{equation}
The non-unitarity $\eta$ of Equation \ref{eqn:deviation_of_unitarity}
consists of four free parameters: mass of heavy vector-like neutrinos $%
M_{44}^{\nu}$, a real number $y$, a CP violation phase $\delta$, and a
Majorana phase $\alpha$. The experimental branching ratio of $\mu
\rightarrow e \gamma$ decay constrains the minimal parameter space in terms
of $M_{44}^{\nu}$ and $y$, while setting up two phases $\delta,\alpha$ which
maximize or minimize the branching ratio of $\mu \rightarrow e \gamma$\cite%
{Hernandez-Garcia:2019uof}, and the minimal parameter space is shown in Figure \ref{fig:parameter_space_muegamma_M44_vu_tanbeta}.
\begin{figure}[H]
\centering
\begin{subfigure}{0.48\textwidth}
	\includegraphics[keepaspectratio,width=\textwidth]{MuegammaNHIH.jpg}
\end{subfigure} \hspace{0.1cm}
\begin{subfigure}{0.48\textwidth}
	\includegraphics[keepaspectratio,width=\textwidth]{MuegammaNHIH11.jpg}
\end{subfigure}
\caption{The left plot is an available parameter space for two free
parameters: mass of vector-like neutrino $M_{44}^{\protect\nu}$ and SM
up-type Higgs vev $v_u$. Here, the free parameter $y$ is set to $1$. The
right plot is the case where vev of the up-type Higgs is constrained from $%
246/\protect\sqrt{2} \simeq 174$ to $246\func{GeV}$ or from $\tan\protect%
\beta = 1$ to $50$ in a same way}
\label{fig:parameter_space_muegamma_M44_vu_tanbeta}
\end{figure}
The left plot in Figure \ref{fig:parameter_space_muegamma_M44_vu_tanbeta} is
an available parameter space for mass of the vector-like neutrino versus the free
parameter $y$ times SM up-type Higgs vev $v_u$. The blue bold line
corresponds to bound of the branching ratio of $\mu \rightarrow e \gamma$
decay at the normal hierarchy with CP violation phase $\delta = 0$ and
Majorana phase $\alpha = 0$ and this line can be relaxed up to the blue
dotted line where $\delta = 0$, $\alpha = 2\pi$. The green bold(dotted) line
corresponds to the inverted hierarchy with $\delta = \pi/2(0)$ and $\alpha = 
\frac{9\pi}{10}(0)$. Since we are especially interested in the range of SM
up-type Higgs vev $v_u$ from $174$ to $246\func{GeV}$, the right plot
consistent with the interested range is extracted from the left after
replacing $v_u$ by $\tan\beta=v_u/v_d$ using the relation $v_u^2 + v_d^2 =
(246 \func{GeV})^2$. \newline
~\newline
As for the constraint of deviation of unitarity $\eta$ with the CLFV $\mu
\rightarrow e \gamma$ decay at $1 \sigma$, it is given by\cite%
{Fernandez-Martinez:2016lgt,Tanabashi:2018oca}
\begin{equation}
\lvert \eta_{21} \rvert \leq 8.4 \times 10^{-6}.
\label{eqn:constraint_nonunitarity_eta21}
\end{equation}

\subsubsection{The muon and electron magnetic moments $\Delta a_{\mu,e}$}

As in the constraint for $\eta_{21}$ in Equation \ref%
{eqn:constraint_nonunitarity_eta21}, the other non-unitarities $\eta_{11,22}$
for the electron and muon anomalous mangetic moment are given by\cite%
{Hernandez-Garcia:2019uof,Fernandez-Martinez:2016lgt}
\begin{equation}
\begin{split}
\eta_{11} &< 4.2 \times 10^{-4} \text{ (for NH) }, \quad < 4.8 \times
10^{-4} \text{ (for IH) } \\
\eta_{22} &< 2.9 \times 10^{-7} \text{ (for NH) }, \quad < 2.4 \times
10^{-7} \text{ (for IH) }  \label{eqn:non_unitarity_eta11_eta_22}
\end{split}%
\end{equation}
With the constraints $\eta_{11,22}$ in Equation \ref%
{eqn:non_unitarity_eta11_eta_22}, we can calculate impact of the muon and
electron anomalous magnetic moments at NH(IH) using Equation \ref%
{eqn:prediction_muegamma_muong2_electrong2}.
\begin{equation}
\begin{split}
\Delta a_\mu &= \frac{\alpha_W}{16\pi} \frac{m_\mu^2}{M_W^2} \eta_{22}
\left( F(x_4) - F(0) \right) \simeq -6.6(-5.5) \times 10^{-16} \\
\Delta a_e &= \frac{\alpha_W}{16\pi} \frac{m_e^2}{M_W^2} \eta_{11} \left(
F(x_4) - F(0) \right) \simeq -2.2(-2.6) \times 10^{-17}
\label{eqn:magnitude_muon_electrong2_with_constraints}
\end{split}%
\end{equation}
There are two interesting features in the above prediction for the muon and
electron anomalous magnetic moments. One feature is sign of each prediction.
As mentioned in the introduction, this prediction with the $W$ exchange can not flip the sign of
each anomaly. In order to explain both anomalies at $1 \sigma$, the
prediction for both anomalies with $W$ exchange requires additional
contributions such as $Z^\prime$ or scalar exchange. Another feature is
magnitude of each prediction. For the muon anomaly, the experimental order
of magnitude at $1 \sigma$ is about $10^{-9}$, however our prediction is
much smaller than that of the experimental bound as well as the electron
anomaly, which means the non-unitarity derived from the presence of heavy
vector-like neutrino can not bring the anomalies to the observable level.
This inadequate prediction with $W$ exchange has been a good motivation to
search for another possibility such as scalar exchange.

\section{Higgs exchange contributions to $(g-2)_\mu, (g-2)_e$ and $\func{BR}\left(\mu \rightarrow e \gamma \right)$} \label{sec:second_paper_Higgs_exchange}

The relevant sector for the muon and electron anomalous magnetic moments with
scalar exchange is charged lepton, so revisit the effective Yukawa matrix
for the charged leptons of Equation \ref%
{eqn:effective_Yukawa_matrix_charged_leptons_assumption}.
\begin{equation}
\begin{split}
y_{ij}^e &= 
\begin{pmatrix}
0 & 0 & 0 \\ 
0 & y_{24}^e x_{42}^{e} & y_{24}^e x_{43}^{e} \\ 
0 & y_{34}^e x_{42}^{e} & y_{34}^e x_{43}^{e}
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{44}^{e}} + 
\begin{pmatrix}
y_{15}^e x_{51}^{e} & y_{15}^e x_{52}^{e} & y_{15}^e x_{53}^{e} \\ 
y_{25}^e x_{51}^{e} & y_{25}^e x_{52}^{e} & y_{25}^e x_{53}^{e} \\ 
y_{35}^e x_{51}^{e} & y_{35}^e x_{52}^{e} & y_{35}^e x_{53}^{e}
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{55}^{e}} \\
&+ 
\begin{pmatrix}
y_{51}^e x_{15}^{L} & y_{52}^e x_{15}^{L} & y_{53}^e x_{15}^{L} \\ 
y_{51}^e x_{25}^{L} & y_{52}^e x_{25}^{L} & y_{53}^e x_{25}^{L} \\ 
y_{51}^e x_{35}^{L} & y_{52}^e x_{35}^{L} & y_{53}^e x_{35}^{L}
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{55}^{L}} + 
\begin{pmatrix}
0 & 0 & 0 \\ 
0 & 0 & 0 \\ 
0 & 0 & x_{34}^L y_{43}^e
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{44}^{L}}
\end{split}
\label{eqn:effective_Yukawa_matrix_charged_leptons_assumption_second}
\end{equation}
The effective Yukawa matrix of Equation \ref%
{eqn:effective_Yukawa_matrix_charged_leptons_assumption_second} in the
mass basis is diagonalized by the universal seesaw mechanism due to involving a
few of different mass scales. Therefore, the only diagonal
components should alive in the mass matrix. In order to make the mass matrix
diagonal, we assume that $y_{34}^e = x_{43}^{e} = y_{15,25,35}^e =
x_{51,52,53}^{e} = x_{25,35}^L = y_{52,53}^e = 0$. Then, the mass matrix is
reduced to
\begin{equation}
\resizebox{\textwidth}{!}{$
\begin{split}
y_{ij}^e &= 
\begin{pmatrix}
0 & 0 & 0 \\ 
0 & y_{24}^e x_{42}^{e} & 0 \\ 
0 & 0 & 0
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{44}^{e}} + 
\begin{pmatrix}
0 & 0 & 0 \\ 
0 & 0 & 0 \\ 
0 & 0 & 0
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{55}^{e}} + 
\begin{pmatrix}
y_{51}^e x_{15}^{L} & 0 & 0 \\ 
0 & 0 & 0 \\ 
0 & 0 & 0
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{55}^{L}} + 
\begin{pmatrix}
0 & 0 & 0 \\ 
0 & 0 & 0 \\ 
0 & 0 & x_{34}^L y_{43}^e
\end{pmatrix}
\frac{\left\langle \phi \right\rangle}{M_{44}^{L}} \\
y_{ij}^e &= 
\begin{pmatrix}
y_{51}^e s_{15}^L & 0 & 0 \\ 
0 & y_{24}^e s_{24}^{e} & 0 \\ 
0 & 0 & y_{43}^e s_{34}^L%
\end{pmatrix},
\label{eqn:diagonalized_Yukawa_matrix_charged_leptons}
\end{split}$}%
\end{equation}
where $s_{15}^L \simeq x_{15}^L \left\langle \phi \right\rangle/M_{55}^{L}$, 
$s_{24}^{e} \simeq x_{42}^{e} \left\langle \phi \right\rangle/M_{44}^{e}$, $%
s_{34}^L \simeq x_{34}^L \left\langle \phi \right\rangle/M_{44}^L$ and the
diagonal elements from top-left to bottom-right should be responsible for
electron, muon and tau Yukawa constants, respectively. After removing all
irrelevant terms to both anomalies and applying the assumption, the $7
\times 7$ mass matrix in the interaction basis is also reduced to as below:
\begin{equation}
M^{e}=\left( 
\begin{array}{c|cccc}
& e_{1R} & e_{2R} & e_{4R} & \widetilde{L}_{5R} \\ \hline
\overline{L}_{1L} & 0 & 0 & 0 & x_{15}^{L}v_{\phi } \\ 
\overline{L}_{2L} & 0 & 0 & y_{24}^{e}v_{d} & 0 \\ 
\overline{L}_{5L} & y_{51}^{e}v_{d} & 0 & 0 & M_{55}^{L} \\ 
\overline{\widetilde{e}}_{4L} & 0 & x_{42}^{e}v_{\phi } & M_{44}^{e} & 0
\end{array}%
\right) \label{eqn:reduced_charged_lepton_mass_matrix}
\end{equation}
The reduced charged lepton mass matrix of Equation \ref%
{eqn:reduced_charged_lepton_mass_matrix} clearly tells
that no mixing between charged leptons arise so the branching ratio of $\mu
\rightarrow e \gamma$ is naturally satisfied under this scenario. The scalar
exchange for both anomalies can be realized by closing the Higgs sectors in
Figure \ref{fig:diagrams_charged_leptons_mass_insertion} as per Figure \ref%
{fig:muon_electrong2_scalar_exchange}.
\begin{figure}[]
\centering
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{muong2_charged_leptons}
\end{subfigure} \hspace{0.1cm}
\begin{subfigure}{0.48\textwidth}
	\includegraphics[width=1.0\textwidth]{electrong2_charged_leptons}
\end{subfigure}
\caption{Diagrams contributing to the muon anomaly (left) and
the electron anomaly (right) where $H_{1,2}$ are CP-even non-SM
scalars and $A_{1,2}$ are CP-odd scalars in the physical basis}
\label{fig:muon_electrong2_scalar_exchange}
\end{figure}
In Figure \ref{fig:muon_electrong2_scalar_exchange}, the CP-even non-SM scalars $%
H_{1,2}$ and CP-odd scalars $A_{1,2}$ appear as a result of mixing between
Higgses $H_u,H_d$ and $\phi$ in the interaction basis. The Higgs sector in the interaction
basis is defined by
\begin{equation}
\begin{split}
H_u &= 
\begin{pmatrix}
H_u^+ \\ 
v_u + \frac{1}{\sqrt{2}}\left( \func{Re}H_{u}^0 + i\func{Im}H_{u}^0 \right)%
\end{pmatrix},%
\\
H_d &= 
\begin{pmatrix}
v_d + \frac{1}{\sqrt{2}}\left( \func{Re}H_{d}^0 + i\func{Im}H_{d}^0 \right)
\\ 
H_d^-%
\end{pmatrix},%
\\ 
\phi &= \frac{1}{\sqrt{2}} \left( v_\phi + \func{Re}\phi + i\func{Im}%
\phi \right).  \label{eqn:Higgs_fields_mass_basis}
\end{split}%
\end{equation}
For consistency, we equate $v_u, v_d$ and $v_\phi$ to $v_1, v_2$ and $v_3$,
respectively.

\subsection{The 2HDM scalar potential} \label{sec:second_paper_scalar_potential}

The scalar potential of the model under
consideation takes the form:%
\begin{equation}
\begin{split}
V =&\mu _{1}^{2}\left( H_{u}H_{u}^{\dagger }\right) +\mu _{2}^{2}\left(
H_{d}H_{d}^{\dagger }\right) +\mu _{3}^{2}\left( \phi \phi ^{\ast }\right)
-\mu _{\func{sb}}^{2}\left[ \phi ^{2}+\left( \phi ^{\ast }\right) ^{2}\right]
+\lambda _{1}\left( H_{u}H_{u}^{\dagger }\right) ^{2}+\lambda _{2}\left(
H_{d}H_{d}^{\dagger }\right) ^{2} \\
&+\lambda _{3}\left( H_{u}H_{u}^{\dagger }\right) \left(
H_{d}H_{d}^{\dagger }\right) +\lambda _{4}\left( H_{u}H_{d}^{\dagger
}\right) \left( H_{d}H_{u}^{\dagger }\right) +\lambda _{5}\left( \varepsilon
_{ij}H_{u}^{i}H_{d}^{j}\phi ^{2}+\func{h.c}\right)  \\
&+\lambda _{6}\left( \phi \phi ^{\ast }\right) ^{2}+\lambda _{7}\left( \phi
\phi ^{\ast }\right) \left( H_{u}H_{u}^{\dagger }\right) +\lambda _{8}\left(
\phi \phi ^{\ast }\right) \left( H_{d}H_{d}^{\dagger }\right) ,
\end{split}
\end{equation}%
where the $\lambda _{i}$ ($i=1,2,\cdots ,8$) are dimensionless parameters
whereas the $\mu _{j}$ ($j=1,2,3$) are dimensionful parameters and $\mu _{%
\func{sb}}$ is a dimensionfull soft-breaking parameter. We consider the $%
U(1)^{\prime }$ symmetry as global in this model so our model does not
feature $Z^{\prime }$ boson and the scalar potential requires the inclusion
of the soft-breaking mass term $-\mu _{\func{sb}}^{2}\left[ \phi ^{2}+\left( \phi
^{\ast }\right) ^{2}\right] $ in order to prevent the appearance of a
massless scalar state arising from the imaginary part of $\phi $.

The minimization conditions of the scalar potential yield the following
relations: 
\begin{equation}
\begin{split}
\mu _{1}^{2} &=-2\lambda _{1}v_{1}^{2}-\lambda _{3}v_{2}^{2}-\frac{1}{2}%
\lambda _{7}v_{3}^{2}-\frac{\lambda _{5}v_{2}v_{3}^{2}}{2v_{1}}, \\
\mu _{2}^{2} &=-\lambda _{3}v_{1}^{2}-\frac{\lambda _{5}v_{3}^{2}v_{1}}{%
2v_{2}}-2\lambda _{2}v_{2}^{2}-\frac{1}{2}\lambda _{8}v_{3}^{2}, \\
\mu _{3}^{2} &=-\lambda _{8}v_{2}^{2}-\lambda _{6}v_{3}^{2}-v_{1}\left(
2\lambda _{5}v_{2}+\lambda _{7}v_{1}\right) -2\mu _{\func{sb}}^{2}.
\end{split}
\end{equation}

\subsection{Mass matrix for CP-even, CP-odd neutral and charged scalars}
\label{subsec:mass_mamtrix_for_CP_even_odd_charged} The squared mass matrix
for the CP-even scalars in the basis $\left( \func{Re}H_{u}^{0},\func{Re}%
H_{d}^{0},\func{Re}\phi \right) $ takes the form:%
\begin{equation}
\mathbf{M}_{\func{CP-even}}^{2}=\left( 
\begin{array}{ccc}
4\lambda _{1}v_{1}^{2}-\frac{\lambda _{5}v_{2}v_{3}^{2}}{2v_{1}} & \frac{1}{2%
}\lambda _{5}v_{3}^{2}+2\lambda _{3}v_{1}v_{2} & \sqrt{2}v_{3}\left( \lambda
_{5}v_{2}+\lambda _{7}v_{1}\right) \\ 
\frac{1}{2}\lambda _{5}v_{3}^{2}+2\lambda _{3}v_{1}v_{2} & 4\lambda
_{2}v_{2}^{2}-\frac{\lambda _{5}v_{1}v_{3}^{2}}{2v_{2}} & \sqrt{2}%
v_{3}\left( \lambda _{5}v_{1}+\lambda _{8}v_{2}\right) \\ 
\sqrt{2}v_{3}\left( \lambda _{5}v_{2}+\lambda _{7}v_{1}\right) & \sqrt{2}%
v_{3}\left( \lambda _{5}v_{1}+\lambda _{8}v_{2}\right) & 2\lambda
_{6}v_{3}^{2}
\end{array}%
\right).  \label{eqn:mass_matrix_CP_even}
\end{equation}
From the mass matrix given above, we find that the CP-even scalar spectrum
is composed of the $125$ GeV\ SM-like Higgs $h$ and two non-SM CP-even
Higgses $H_{1,2}$. Furthermore, we assume that no mixing between the SM
physical Higgs $h$ and the two non-SM CP-even Higgses $H_{1,2}$ arise and
this assumption constrains the $(1,2)$, $(1,3)$, $(2,1)$ and $(3,1)$ elements of
CP-even mass matrix of Equation \ref{eqn:mass_matrix_CP_even}. The
constraints are given by the following decoupling limit scenario
\begin{equation}
\begin{split}
\lambda_5 &= \frac{-4 v_1 v_2}{v_3^2} \lambda_3 \\
\lambda_7 &= -\frac{v_2}{v_1} \lambda_5 = \frac{4 v_2^2}{v_3^2} \lambda_3,
\label{eqn:constraints_in_mass_matrix_CP_even}
\end{split}%
\end{equation}
and then the CP-even mass matrix of Equation \ref{eqn:mass_matrix_CP_even}
with the constraints is simplified to
\begin{equation}
\mathbf{M}_{\func{CP-even}}^{2}=\left( 
\begin{array}{ccc}
4\lambda _{1}v_{1}^{2} + 2v_{2}^{2} \lambda_{3} & 0 & 0 \\ 
0 & 4\lambda _{2}v_{2}^{2} + 2v_{1}^{2} \lambda_{3} & \sqrt{2}v_{3}\left( -%
\frac{4 v_{1}^{2} v_{2}}{v_{3}^{2}} \lambda_{3} +\lambda _{8}v_{2}\right) \\ 
0 & \sqrt{2}v_{3}\left( -\frac{4 v_{1}^{2} v_{2}}{v_{3}^{2}} \lambda_{3}
+\lambda _{8}v_{2}\right) & 2\lambda _{6}v_{3}^{2}%
\end{array}%
\right).  \label{eqn:mass_matrix_CP_even_simplified}
\end{equation}
In the above given decoupling limit scenario, chosen in order to simplify our analysis, 
%we will restrict to the scenario of the decoupling limit where 
the CP-even neutral scalar states contained in the $SU(2)$
doublet $H_{u}$ will not mix with the CP-even neutral ones contained in $%
H_{d}$. In such limit, the neutral CP-even states of $H_{u}$ will not
feature mixing with the gauge singlet scalar $\phi $. Thus, the lightest $125%
\func{GeV}$ CP-even scalar of our model will have couplings to the SM
particles close to the SM expectation, which is consistent with the current
experimental data.

Diagonalizing the simplified CP-even mass matrix, it reveals masses of the
physical SM Higgs $h$ and non-SM CP-even scalars $H_{1,2}$ in the physical
basis $\left( h, H_1, H_2 \right)$
\begin{equation}
R_{\func{CP-even}}^\dagger \mathbf{M}_{\func{CP-even}}^2 R_{\func{CP-even}}
= \func{diag} \left( m_h^2, m_{H_1}^2, m_{H_2}^2 \right).
\label{eqn:diagonalising_CP_even_mass_matrix}
\end{equation}
The SM Higgs $h$ is appeared as $\func{Re}H_{u}^{0}$ itself and the non-SM
CP-even scalars $H_{1,2}$ are the states which $\func{Re}H_{d}^{0}$ is mixed
with $\func{Re}\phi $. Regarding the CP-odd scalar sector, we find that the
squared mass matrix for the CP-odd scalars in the basis $\left( \func{Im}%
H_{u}^{0},\func{Im}H_{d}^{0},\func{Im}\phi \right) $ is given by: 
\begin{equation}
\mathbf{M}_{\func{CP-odd}}^{2}=\left( 
\begin{array}{ccc}
-\frac{\lambda _{5}v_{2}v_{3}^{2}}{2v_{1}} & -\frac{1}{2}\lambda
_{5}v_{3}^{2} & -\sqrt{2}\lambda _{5}v_{2}v_{3} \\ 
-\frac{1}{2}\lambda _{5}v_{3}^{2} & -\frac{\lambda _{5}v_{1}v_{3}^{2}}{2v_{2}%
} & -\sqrt{2}\lambda _{5}v_{1}v_{3} \\ 
-\sqrt{2}\lambda _{5}v_{2}v_{3} & -\sqrt{2}\lambda _{5}v_{1}v_{3} & 
-4\lambda _{5}v_{1}v_{2}-4\mu _{\func{sb}}^{2}%
\end{array}%
\right).
\end{equation}
The squared CP-odd mass matrix is diagonalized in the same way as in the
CP-even mass matrix and the CP-odd physical basis is given by $\left(
G_{Z},A_{1},A_{2}\right) $ where $G_{Z}$ is the massless Goldstone bosons
associated with the longitudinal components of the $Z$ gauge boson, whereas $%
A_{1}$ and $A_{2}$ are massive non-SM CP-odd scalars
\begin{equation}
R_{\func{CP-odd}}^{\dagger }\mathbf{M}_{\func{CP-odd}}^{2}R_{\func{CP-odd}}=%
\func{diag}\left( 0,m_{A_{1}}^{2},m_{A_{2}}^{2}\right) .
\label{eqn:diagonalizing_CP_odd_mass_matrix}
\end{equation}
Furthermore, the squared mass matrix for the electrically charged scalars is
given by: 
\begin{equation}
\mathbf{M}_{\func{charged}}^{2}=\left( 
\begin{array}{cc}
\lambda _4 v_2^2-\frac{\lambda _5 v_2 v_3^2}{2 v_1} & \lambda _4 v_1 v_2-%
\frac{1}{2} \lambda _5 v_3^2 \\ 
\lambda _4 v_1 v_2-\frac{1}{2} \lambda _5 v_3^2 & \lambda _4 v_1^2-\frac{%
\lambda _5 v_1 v_3^2}{2 v_2}%
\end{array}
\right).
\end{equation}
The charged scalar mass matrix can be diagonalized in the basis $\left(
H_{1}^{\pm}, H_{2}^{\pm} \right)$ as in CP-even or -odd mass matrix:
\begin{equation}
R_{\func{charged}}^\dagger \mathbf{M}_{\func{charged}}^{2} R_{\func{charged}%
} = \func{diag} \left( 0, m_{H^\pm}^2 \right).
\label{eqn:diagonalizing_charged_mass_matrix}
\end{equation}
Then, the electrically charged scalar sector contains the massive scalars $%
H^{\pm }$ and the massless electrically charged scalars $G_{W}^{\pm }$ which
correspond to the Goldstone bosons associated with the longitudinal
components of the $W^{\pm }$ gauge bosons. In the following sections we will
analyze the phenomenological implications of our model in the Higgs diphoton
decay as well as in the muon and electron anomalous magnetic moments. 

\subsection{The Higgs diphoton signal strength} \label{sec:second_paper_hphopho}

The rate for the $h\rightarrow \gamma \gamma $ decay is
given by: 
\begin{equation}
\Gamma (h\rightarrow \gamma \gamma )=\dfrac{\alpha _{\func{em}}^{2}m_{h}^{3}%
}{256\pi ^{3}v^{2}}\left\vert \sum_{f}a_{hff}N_{C}Q_{f}^{2}F_{1/2}(\rho
_{f})+a_{hWW}F_{1}(\rho _{W})+\frac{C_{hH^{\pm }H^{\mp }}v}{2m_{H^{\pm }}^{2}%
}F_{0}(\rho _{H_{k}^{\pm }})\right\vert ^{2},
\end{equation}%
where $\rho _{i}$ are the mass ratios $\rho _{i}=\frac{m_{h}^{2}}{4M_{i}^{2}}
$ with $M_{i}=m_{f},M_{W}$; $\alpha _{\func{em}}$ is the fine structure
constant; $N_{C}$ is the color factor ($N_{C}=1$ for leptons and $N_{C}=3$
for quarks) and $Q_{f}$ is the electric charge of the fermion in the loop.
From the fermion-loop contributions we only consider the dominant top quark
term. Furthermore, $C_{hH^{\pm }H^{\mp }}$ is the trilinear coupling between
the SM-like Higgs and a pair of charged Higges, whereas $a_{htt}$ and $%
a_{hWW}$ are the deviation factors from the SM Higgs-top quark coupling and
the SM Higgs-W gauge boson coupling, respectively (in the SM these factors
are unity). Such deviation factors are close to unity in our model and they
are defined as below:
\begin{equation}
a_{htt} \simeq 1, \quad a_{hWW} = \frac{1}{\sqrt{v_1^2 + v_2^2}} \frac{%
\partial}{\partial h} \left( \sum_{i,j=1,2,3} v_i \left( R_{\func{CP-even}%
}^T \right)_{ij} \left( h, H_1, H_2 \right)_{j} \right) = \frac{v_1}{\sqrt{%
v_1^2 + v_2^2}}
\end{equation}
Furthermore, $F_{1/2}(z)$ and $F_{1}(z)$ are the dimensionless loop factors
for spin-$1/2$ and spin-$1$ particles running in the internal lines of the
loops. These loop factors take the form:
\begin{equation}
\begin{split}
F_{1/2}(z)& =2(z+(z-1)f(z))z^{-2}, \\
F_{1}(z)& =-2(2z^{2}+3z+3(2z-1)f(z))z^{-2}, \\
F_{0}(z)& =-(z-f(z))z^{-2},
\end{split}%
\end{equation}%
with 
\begin{equation}
f(z)=\left\{ 
\begin{array}{lcc}
\arcsin ^{2}\sqrt{2} & \text{for} & z\leq 1 \\ 
&  &  \\ 
-\frac{1}{4}\left( \ln \left( \frac{1+\sqrt{1-z^{-1}}}{1-\sqrt{1-z^{-1}}%
-i\pi }\right) ^{2}\right) & \text{for} & z>1
\end{array}%
\right.
\end{equation}
In order to study the implications of our model in the decay of the $125$
GeV Higgs into a photon pair, one introduces the Higgs diphoton signal
strength $R_{\gamma \gamma }$, which is defined as: 
\begin{equation}
R_{\gamma \gamma }=\frac{\sigma (pp\rightarrow h)\Gamma (h\rightarrow \gamma
\gamma )}{\sigma (pp\rightarrow h)_{\func{SM}}\Gamma (h\rightarrow \gamma
\gamma )_{\func{SM}}}\simeq a_{htt}^{2}\frac{\Gamma (h\rightarrow \gamma
\gamma )}{\Gamma (h\rightarrow \gamma \gamma )_{\func{SM}}}.  \label{eqn:hgg}
\end{equation}%
That Higgs diphoton signal strength, normalizes the $\gamma \gamma $ signal
predicted by our model in relation to the one given by the SM. Here we have
used the fact that in our model, single Higgs production is also dominated
by gluon fusion as in the Standard Model.

The ratio $R_{\gamma \gamma }$ has been measured by CMS and ATLAS
collaborations with the best fit signals \cite{Sirunyan:2018ouh,Aad:2019mbh}%
: 
\begin{equation}
R_{\gamma \gamma }^{\func{CMS}}=1.18_{-0.14}^{+0.17}\quad \text{and}\quad R_{\gamma
\gamma }^{\func{ATLAS}}=0.96\pm 0.14.  \label{eqn:rgg}
\end{equation}
As it will be shown in the next subsection, the constraints arising from the Higgs diphoton decay rate will be considered in our numerical analysis. %and will restrict the model parameter space.

\subsection{The muon and electron anomalous magnetic moments}
\label{sec:second_paper_mueg2}

The Yukawa interactions relevant for the computation of the muon anomalous
magnetic moment are:
% \begin{equation}
% \begin{split}
% \mathcal{L}_{\Delta a_\mu} &= y_{24}^e L_{2L} \widetilde{H}_d^\dagger 
% \overline{e}_{4R} + M_{44}^{e} \widetilde{e}_{4L} \overline{e}_{4R} +
% x_{42}^e \phi \widetilde{e}_{4L} \overline{e}_{2R} + \func{h.c.} \\
% &= y_{24}^e \mu_L H_d^0 \overline{e}_{4R} + M_{44}^e \widetilde{e}_{4L} 
% \overline{e}_{4R} + x_{42}^e \phi \widetilde{e}_{4L} \overline{e}_{2R} +
% \cdots + \func{h.c.}
% \end{split}
% \label{eqn:Lagrangian_muon_anomaly_left_handed}
% \end{equation}
%
% The Lagrangian of Equation \ref%
% {eqn:Lagrangian_muon_anomaly_right_handed} is not allowed to write in our
% mass matrix since we have turned off the interactions by rotating the
% charged lepton mass matrix of Equation \ref%
% {eqn:a_specified_basis_charged_leptons_second}, however it gives totally same
% theoretical prediction for muon anomaly as the above Lagrangian so we allow
% them to be written in order to arrive to the CP-even(odd) scalar mass basis.
%
% \begin{equation}
% \mathcal{L}_{\Delta a_\mu} = y_{24}^{e *} \mu_{R} \widetilde{H}_d^{0 *} 
% \overline{e}_{4R} + M_{44}^{e} \widetilde{e}_{4R} \overline{e}_{4L} +
% x_{42}^{e *} \phi^* \widetilde{e}_{4R} \overline{e}_{2L} + \cdots + \func{%
% h.c.}  \label{eqn:Lagrangian_muon_anomaly_right_handed}
% \end{equation}
%
% Adding Equation \ref{eqn:Lagrangian_muon_anomaly_left_handed} to \ref%
% {eqn:Lagrangian_muon_anomaly_right_handed} while assuming the coupling
% constants $y_{24}^e,x_{42}^e$ are real and expanding the scalars by the real
% and imaginary parts with the projection operators $P_{L,R}$ taken out from
% the charged leptons, we have
\begin{equation}
\mathcal{L}_{\Delta a_\mu} = y_{24}^e \mu \left( \func{Re} H_{d}^0 - i
\gamma^5 \func{Im} H_{d}^0 \right) \overline{e}_4 + x_{42}^e \widetilde{e}_4
\left( \func{Re} \phi - i \gamma^5 \func{Im} \phi \right) \overline{e}_2 +
M_{44}^e \widetilde{e}_4 \overline{e}_4 + \func{h.c.}
\label{eqn:Lagrangian_muon_anomaly_expansion}
\end{equation}
where the Yukawa coupling constants $y_{24}^e,x_{42}^e$ are assumed to be real, the scalar fieds have been expanded by their real and imaginary parts and the properties of the projection operators $P_{L,R}$ acting on the charged leptonic fields have been used.
%Using the mixing between scalars
By expressing the scalar fields in the interaction basis in terms of the scalar fields in the physical basis, the charged lepton Yukawa interactions relevant for the computation of the $g-2$ anomalies take the form:
%the final Lagrangian for the muon anomalous magnetic moment is
\begin{equation}
\begin{split}
\mathcal{L}_{\Delta a_{\mu }}& =y_{24}^{e}\mu \left(
(R_{e}^{T})_{22}H_{1}+(R_{e}^{T})_{23}H_{2}-i\gamma
^{5}(R_{o}^{T})_{22}A_{1}-i\gamma ^{5}(R_{o}^{T})_{23}A_{2}\right) \overline{%
e}_{4} \\
& +x_{42}^{e}\widetilde{e}_{4}\left(
(R_{e}^{T})_{32}H_{1}+(R_{e}^{T})_{33}H_{2}-i\gamma ^{5}( R_{o}^{T})
_{32}A_{1}-i\gamma ^{5}(R_{o}^{T})_{33}A_{2}\right) \overline{e}%
_{2}+M_{44}^{e}\widetilde{e}_{4}\overline{e}_{4}+\func{h.c.}
\end{split}%
\end{equation}
where we are using the unitary gauge where the contributions arising from
unphysical Goldstone bosons to the muon anomaly are excluded and we shorten
the notations $R_{\func{CP}}$ by $R_{e(o)}$. Here $R_{e}$ and $R_{o}$ are the rotation matrices that diagonalize the squared mass matrices for the CP even and CP odd scalars, respectively. Then, it follows that the muon and electron anomalous magnetic moments in the scenario of diagonal SM charged lepton mass matrix take the form:
\begin{equation}
\begin{split}
\Delta a_{\mu }=y_{24}^{e}x_{42}^{e}\frac{m_{\mu }^{2}}{8\pi ^{2}}\Big[&
\left( R_{e}^{T}\right) _{22}\left( R_{e}^{T}\right) _{32}I_{S}^{(\mu
)}\left( m_{e_{4}},m_{H_{1}}\right) +\left( R_{e}^{T}\right) _{23}\left(
R_{e}^{T}\right) _{33}I_{S}^{(\mu )}\left( m_{e_{4}},m_{H_{2}}\right) \\
& -\left( R_{o}^{T}\right) _{22}\left( R_{o}^{T}\right) _{32}I_{P}^{(\mu
)}\left( m_{e_{4}},m_{A_{1}}\right) -\left( R_{o}^{T}\right) _{23}\left(
R_{o}^{T}\right) _{33}I_{P}^{\left( \mu \right) }\left(
m_{e_{4},}m_{A_{2}}\right) \Big] \\
\Delta a_{e}=y_{51}^{e}x_{15}^{L}\frac{m_{e}^{2}}{8\pi ^{2}}\Big[& \left(
R_{e}^{T}\right) _{22}\left( R_{e}^{T}\right) _{32}I_{S}^{(e)}\left(
m_{e_{5}},m_{H_{1}}\right) +\left( R_{e}^{T}\right) _{23}\left(
R_{e}^{T}\right) _{33}I_{S}^{(e)}\left( m_{e_{5}},m_{H_{2}}\right) \\
& -\left( R_{o}^{T}\right) _{22}\left( R_{o}^{T}\right)
_{32}I_{P}^{(e)}\left( m_{e_{5}},m_{A_{1}}\right) -\left( R_{o}^{T}\right)
_{23}\left( R_{e}^{T}\right) _{33}I_{P}^{\left( E\right) }\left(
m_{e_{5}},m_{A_{2}}\right) \Big],
\end{split}
\label{eqn:muon_electron_anomalous_magnetic_moments}
\end{equation}
where the loop integrals are given by \cite{Diaz:2002uk,Jegerlehner:2009ry,Kelso:2014qka,Lindner:2016bgg,Kowalska:2017iqv}: 
\begin{equation}
I_{S\left( P\right) }^{\left( e,\mu \right) }\left( m_{E_{4,5}},m_{S}\right)
=\int_{0}^{1}\frac{x^{2}\left( 1-x\pm \frac{m_{E_{4,5}}}{m_{e,\mu }}\right) }{%
m_{e,\mu }^{2}x^{2}+\left( m_{E_{4,5}}^{2}-m_{e,\mu }^{2}\right) x+m_{S,P}^{2}\left(
1-x\right) }dx  \label{eqn:loop_integrals}
\end{equation}
and $S(P)$ means scalar (pseudoscalar) and $E_{4,5}$ stands for the vector-like family. It is worth mentioning that $E_{4}$ and $E_{5}$ only contribute to the muon and electron anomalous magnetic moments, respectively.

\section{Numerical analysis of the Higgs exchange contributions} \label{sec:second_paper_numeric_Higgs}

For the sake of simplicity, we consider the scenario of absence of mixing between SM charged leptons, which automatically prevents charged lepton flavour violating decays.   
%We assumed no mixing between charged leptons arise. Therefore, our model
%does not feature charged lepton flavour violating decays. %In our numerical
%analysis of the scalar sector, we have found that the CP-odd neutral and
%electrically charged scalars have masses close to about $800 \func{GeV}$ and 
%$1 \func{TeV}$, respectively. 
In our numerical analysis we have
found that the non-SM CP-even scalar mass can reach values around $200 \func{%
GeV}$. Despite the fact that the non SM CP-even scalar is quite light and can have
a sizeable decay mode into a bottom-anti bottom quark pair, its single LHC
production via gluon fusion mechanism is strongly suppressed since it is
dominated by the triangular bottom quark loop. Such non SM CP-even scalar $H$
can also be produced by vector boson fusion but such production is expected
to have a low total cross section due to small $HWW$ and $HZZ$ couplings,
which are proportional to $v_d$. In this section we will discuss the
implications of our model in the muon and electron anomalous magnetic
moments.

\subsection{The fitting function $\chi^2$ and free parameter setup} \label{sec:second_paper_chi2}

For the first approach to both anomalies, we construct the fitting function $%
\chi^2$
\begin{equation}
\begin{split}
\chi^2 &= \frac{\left( m_h^{\func{Thy}}-m_h^{\func{Cen}} \right)^2}{\left(
\delta m_h^{\func{Dev}} \right)^2} + \frac{\left( a_{hWW}^{\func{Thy}%
}-a_{hWW}^{\func{Cen}} \right)^2}{\left( \delta a_{hWW}^{\func{Dev}}
\right)^2} + \frac{\left( R_{\gamma\gamma}^{\func{Thy}}-R_{\gamma\gamma}^{%
\func{Cen}} \right)^2}{\left( \delta R_{\gamma\gamma}^{\func{Dev}} \right)^2}
\\
&+ \frac{\left( \Delta a_{\mu}^{\func{Thy}}-\Delta a_{\mu}^{\func{Cen}}
\right)^2}{\left( \delta \Delta a_{\mu}^{\func{Dev}} \right)^2} + \frac{%
\left( \Delta a_{e}^{\func{Thy}}-\Delta a_{e}^{\func{Cen}} \right)^2}{\left(
\delta \Delta a_{e}^{\func{Dev}} \right)^2},
\end{split}%
\end{equation}
where the superscripts $\func{Thy}$, $\func{Cen}$ and $\func{Dev}$ mean
theoretical prediction, central value of experimental bound and deviation
from the central value at one of $1,2,3\sigma$, respectively. The parameters
used in this fitting function are defined as below(the integer number
multiplied in delta terms means $\sigma$):
\begin{equation}
\begin{split}
m_h^{\func{Cen}} = 125.38 \func{GeV}, &\quad \delta m_h^{\func{Dev}} = 3
\times 0.14 \func{GeV}, \\
a_{hWW}^{\func{Cen}} = 0.59, &\quad \delta a_{hWW}^{\func{Dev}} = 1 \times
0.35, \\
R_{\gamma \gamma}^{\func{Cen}} = \frac{1}{2} \left( R_{\gamma \gamma}^{\func{%
CMS}} + R_{\gamma \gamma}^{\func{ATLAS}} \right) = 1.07, &\quad \delta
R_{\gamma \gamma}^{\func{Dev}} = 1 \times 0.14, \\
\Delta a_\mu^{\func{Cen}} = 26.1 \times 10^{-10}, &\quad \delta\Delta a_\mu^{%
\func{Dev}} = 1 \times \left( 8.0 \times 10^{-10} \right) \\
\Delta a_e^{\func{Cen}} = -0.88 \times 10^{-12}, &\quad \delta\Delta a_e^{%
\func{Dev}} = 2 \times \left( 0.36 \times 10^{-12} \right)
\end{split}%
\end{equation}
For an initial scan, we set up the starting parameter region as below:
\begin{center}
{\renewcommand{\arraystretch}{1.5} 
\begin{tabular}{|c|c|}
\hline
\textbf{Parameter} & \textbf{Value/Scanned Region($\func{GeV}$)} \\ \hline
$v_u = v_1$ & $\frac{\tan\beta}{\sqrt{1+\tan\beta^2}} \times 246$ \\ 
$v_d = v_2$ & $\frac{1}{\sqrt{1+\tan\beta^2}} \times 246$ \\ 
$v_\phi = v_3$ & $\pm [0.01,1.00] \times 1000$ \\ \hline
$\tan\beta = v_u/v_d$ & $\left[ 5, 50 \right]$ \\ \hline
$\lambda_1$ & $\left( m_h^2 + \frac{v_2 v_3^2 \lambda_5}{2 v_1}
\right)/\left( 4 v_1^2 \right)$ \\ 
$\lambda_2$ & $\pm \left[ 0.50, 12.00 \right]$ \\ 
$\lambda_3$ & $\pm \left[ 0.50, 12.00 \right]$ \\ 
$\lambda_4$ & $\pm \left[ 0.50, 12.00 \right]$ \\ 
$\lambda_5$ & $-4 v_1 v_2 \lambda_3/(v_3)^2$ \\ 
$\lambda_6$ & $\pm \left[ 0.50, 12.00 \right]$ \\ 
$\lambda_7$ & $-v_2 \lambda_5/v_1$ \\ 
$\lambda_8$ & $\pm \left[ 0.50, 12.00 \right]$ \\ \hline
$M_{44}^{e}$ & $\left[ 2 \times 10^2, 2 \times 10^3 \right]$ \\ 
$M_{55}^{L}$ & $\left[ 2 \times 10^2, 2 \times 10^3 \right]$ \\ 
$\mu_{\func{sb}}$ & $i^{[0,1]} \times \left[300, 500 \right]$ \\ \hline
$y_{e}$ & $\sqrt{2} m_{e}/v_2$ \\ 
$y_{\mu}$ & $\sqrt{2} m_{\mu}/v_2$ \\ 
$y_{24}^{e}$ & $\pm \left[ 1.0, 3.5 \right]$ \\ 
$y_{51}^{e}$ & $\pm \left[ 1.0, 3.5 \right]$ \\ 
$x_{42}^{e}$ & $\lvert y_{\mu} M_{44}^{e} / \left( y_{24}^{e} v_3 \right)
\rvert$ \\ 
$x_{15}^{L}$ & $\lvert y_{e} M_{55}^{L} / \left( y_{51}^{e} v_3 \right)
\rvert$ \\ \hline
\end{tabular}
\captionof{table}{Initial parameter setup} \label%
{tab:parameter_region_initial_scan}}
\end{center}
\begin{enumerate}
\item For the Higgs vevs, we are interested in the range of $\tan\beta$ from 
$5$ to $50$ as in the $W$ boson exchange in Figure \ref%
{fig:parameter_space_muegamma_M44_vu_tanbeta}

\item For $\lambda_1$, we fixed mass of the SM physical Higgs $h$ to be $125%
\func{GeV}$ to save time and to make the calculation faster. For $%
\lambda_{5,7} $, the assumption that no mixing between the SM Higgs $h$ and
non-SM Higgses $H_{1,2}$ arise is reflected on these parameters. The other
quartic coupling constants $\lambda_{2,3,4,6,8}$ are set up not to go over $%
4\pi$ for perturbativity.

\item For the vector-like masses $M_{44}^{e}$ and $M_{55}^{L}$, there is a
constraint that the lightest should be greater than $200\func{GeV}$ \cite%
{Xu:2018pnq}.

\item In our numerical analysis we consider solutions where the non SM
scalar masses are larger than about $200\func{GeV}$ as done in \cite%
{Hernandez-Sanchez:2020vax}.

\item The soft-breaking mass term $\mu_{\func{sb}}$ is a free parameter,
which does not generate any problem and appropiate values of this parameters
yields masses for scalars and vector-like fermions consistent with the
experimental constraints. 
% as long as this model yields appropriate masses for scalars and vector-like fermions.

\item The diagonal Yukawa constants appearing in Equation \ref%
{eqn:diagonalized_Yukawa_matrix_charged_leptons} should be the Yukawa
constant for electron, muon and tau, respectively. The Yukawa constants $%
y_{24,51}$ and $x_{42,15}$ interacting with vector-like families are defined
under this consideration. For perturbativity, the Yukawa constants $%
y_{24,51} $ are considered not to go over $\sqrt{4\pi}$.
\end{enumerate}

After saturating value of the $\chi^2$ function less than or nearly $2$
which we believe it is converged enough, we find a best peaked value for
each free parameter. For the given parameters, we rename them by adding an
index ``p" to the end of subscript of each parameter like $\func{\tan\beta_p}
$ and then the expansion factor $\kappa$ is multiplied to find a correlation
between the observables and the mass parameters. Then, the parameter region
is refreshed by both the specific value of each parameter and the expansion
factor $\kappa$ as per Table \ref{tab:parameter_region_subsequent_scan}.
\begin{center}
{\renewcommand{\arraystretch}{1.5} 
\begin{tabular}{|c|c|}
\hline
\textbf{Parameter} & \textbf{Value/Scanned Region($\func{GeV}$)} \\ \hline
$v_u = v_1$ & $\frac{\tan\beta_p}{\sqrt{1+\tan\beta_p^2}} \times 246$ \\ 
$v_d = v_2$ & $\frac{1}{\sqrt{1+\tan\beta_p^2}} \times 246$ \\ 
$v_\phi = v_3$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times v_{3p}$
\\ \hline
$\tan\beta = v_u/v_d$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times 
\func{\tan\beta}_p$ \\ \hline
$\lambda_1$ & $\left( m_h^2 + \frac{v_{2} v_{3}^2 \lambda_{5}}{2 v_{1}}
\right)/\left( 4 v_{1}^2 \right)$ \\ 
$\lambda_2$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times \lambda_{2p}$
\\ 
$\lambda_3$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times \lambda_{3p}$
\\ 
$\lambda_4$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times \lambda_{4p}$
\\ 
$\lambda_5$ & $-4 v_{1} v_{2} \lambda_{3}/(v_{3})^2$ \\ 
$\lambda_6$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times \lambda_{6p}$
\\ 
$\lambda_7$ & $-v_{2} \lambda_{5}/v_{1}$ \\ 
$\lambda_8$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times \lambda_{8p}$
\\ \hline
$M_{44}^{e}$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times M_{44p}^{e}$
\\ 
$M_{55}^{L}$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times M_{55p}^{L}$
\\ 
$\mu_{\func{sb}}$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times \mu_{%
\func{sb}p}$ \\ \hline
$y_{e}$ & $\sqrt{2} m_{e}/v_{2}$ \\ 
$y_{\mu}$ & $\sqrt{2} m_{\mu}/v_{2}$ \\ 
$y_{24}^{e}$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times y_{24p}^{e}$
\\ 
$y_{51}^{e}$ & $\left[ (1 - \kappa), (1 + \kappa) \right] \times y_{51p}^{e}$
\\ 
$x_{42}^{e}$ & $y_{\mu} M_{44}^{e} / \left( y_{24}^{e} v_3 \right)$ \\ 
$x_{15}^{L}$ & $y_{e} M_{55}^{L} / \left( y_{51}^{e} v_3 \right)$ \\ \hline
$\kappa$ & $0.1$ \\ \hline
\end{tabular}
\captionof{table}{Next parameter setup after the initial scan result} \label%
{tab:parameter_region_subsequent_scan}}
\end{center}

\subsection{A scanned result on the free parameters as well as observables across over the first and second scan} \label{sec:second_paper_scanned_result}

The best peaked value for each parameter is listed in Table \ref%
{tab:parameter_region_best_peaked} and energy scale is in unit of $\func{GeV}
$. Note that all cases are carried out independently and all points of plots
in each case are collected within $1\sigma$ constraint of each anomaly.

\begin{center}
{\renewcommand{\arraystretch}{1.5} 
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Parameter} & case A & case B & case C & case D \\ \hline
$v_u = v_1$ & $245.925$ & $245.936$ & $245.951$ & $245.917$ \\ 
$v_d = v_2$ & $6.086$ & $5.595$ & $4.921$ & $6.387$ \\ 
$v_\phi = v_3$ & $-57.761$ & $-36.470$ & $-57.919$ & $-30.746$ \\ \hline
$\tan\beta = v_u/v_d$ & $40.410$ & $43.957$ & $49.977$ & $38.503$ \\ \hline
$\lambda_1$ & $0.063$ & $0.064$ & $0.066$ & $0.064$ \\ 
$\lambda_2$ & $-7.978$ & $8.414$ & $-2.000$ & $2.948$ \\ 
$\lambda_3$ & $6.344$ & $2.675$ & $-6.242$ & $1.724$ \\ 
$\lambda_4$ & $1.859$ & $2.158$ & $-3.633$ & $10.837$ \\ 
$\lambda_5$ & $-11.384$ & $-11.070$ & $-9.009$ & $-11.460$ \\ 
$\lambda_6$ & $2.888$ & $1.228$ & $0.866$ & $1.351$ \\ 
$\lambda_7$ & $0.282$ & $0.252$ & $-0.180$ & $0.298$ \\ 
$\lambda_8$ & $-1.363$ & $-1.346$ & $-10.845$ & $-11.510$ \\ \hline
$M_{44}^{e}$ & $1475.010$ & $1355.470$ & $1495.770$ & $1134.340$ \\ 
$M_{55}^{L}$ & $279.386$ & $211.263$ & $204.706$ & $323.292$ \\ 
$\mu_{\func{sb}}$ & $424.618i$ & $443.435i$ & $480.993$ & $480.062i$ \\ 
\hline
$y_{e} \left[ 10^{-4} \right]$ & $1.135$ & $1.234$ & $1.403$ & $1.081$ \\ 
$y_{\mu} \left[ 10^{-2} \right]$ & $2.391$ & $2.600$ & $2.956$ & $2.278$ \\ 
$y_{24}^{e}$ & $-3.161$ & $-3.101$ & $-2.942$ & $-1.548$ \\ 
$y_{51}^{e}$ & $2.315$ & $2.164$ & $2.050$ & $1.352$ \\ 
$x_{42}^{e}$ & $0.193$ & $0.312$ & $0.260$ & $0.543$ \\ 
$x_{15}^{L} \left[ 10^{-4} \right]$ & $2.371$ & $3.304$ & $2.419$ & $8.408$
\\ \hline
$m_{H_1}$ & $213.390$ & $222.924$ & $212.147$ & $238.523$ \\ 
$m_{H_2}$ & $911.585$ & $614.516$ & $891.413$ & $518.147$ \\ 
$m_{A_1}$ & $741.343$ & $537.111$ & $807.268$ & $435.887$ \\ 
$m_{A_2}$ & $1003.790$ & $939.553$ & $1035.800$ & $1006.240$ \\ 
$m_{H^\pm}$ & $938.259$ & $674.054$ & $987.625$ & $929.786$ \\ \hline
$\Delta a_\mu \left[ 10^{-9} \right]$ & $2.734$ & $2.688$ & $2.935$ & $2.891$
\\ 
$\Delta a_e \left[ 10^{-13} \right]$ & $-5.073$ & $-8.310$ & $-5.543$ & $%
-6.365$ \\ 
$a_{hWW}$ & $1.000$ & $1.000$ & $1.000$ & $1.000$ \\ 
$R_{\gamma\gamma}$ & $0.999$ & $0.999$ & $0.999$ & $0.999$ \\ \hline
$\chi^2$ & $1.794$ & $1.516$ & $1.870$ & $1.740$ \\ \hline
\end{tabular}
\captionof{table}{A best peaked value for each parameter at each case. All
energy scale is in unit of $\func{GeV}$} \label{tab:parameter_region_best_peaked}}
\end{center}

Here, we put two constraints on the lightest vector-like mass and the
lightest non-SM scalar mass; the vector-like mass should be greater than $200%
\func{GeV}$ as well as the non-SM scalar mass\cite{Xu:2018pnq,Hernandez-Sanchez:2020vax}. After we
carry out second parameter scan based on the first scan result of Table \ref%
{tab:parameter_region_best_peaked}, range of the parameters are given in
Table \ref{tab:range_secondscan}.

\begin{center}
{\renewcommand{\arraystretch}{1.5} 
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Parameter} & case A & case B & case C & case D \\ \hline
$v_u = v_1$ & $\left[ 245.907 \rightarrow 245.938 \right]$ & $\left[ 245.921
\rightarrow 245.947 \right]$ & $\left[ 245.939 \rightarrow 245.959 \right]$
& $\left[ 245.898 \rightarrow 245.931 \right]$ \\ 
$v_d = v_2$ & $\left[ 5.533 \rightarrow 6.761 \right]$ & $\left[ 5.087
\rightarrow 6.216 \right]$ & $\left[ 4.474 \rightarrow 5.468 \right]$ & $%
\left[ 5.807 \rightarrow 7.096 \right]$ \\ 
$v_\phi = v_3$ & $\left[ -63.525 \rightarrow -51.985 \right]$ & $\left[
-40.117 \rightarrow -32.823 \right]$ & $\left[ -63.706 \rightarrow -52.128 %
\right]$ & $\left[ -33.820 \rightarrow -27.671 \right]$ \\ \hline
$\tan\beta = v_u/v_d$ & $\left[ 36.371 \rightarrow 44.451 \right]$ & $\left[
39.561 \rightarrow 48.353 \right]$ & $\left[ 44.980 \rightarrow 54.975 %
\right]$ & $\left[ 34.653 \rightarrow 42.354 \right]$ \\ \hline
$m_{H_1}$ & $\left[ 200.000 \rightarrow 242.653 \right]$ & $\left[ 201.520
\rightarrow 246.046 \right]$ & $\left[ 200.000 \rightarrow 230.754 \right]$
& $\left[ 215.523 \rightarrow 261.920 \right]$ \\ 
$m_{H_2}$ & $\left[ 752.061 \rightarrow 1088.130 \right]$ & $\left[ 516.289
\rightarrow 724.997 \right]$ & $\left[ 735.831 \rightarrow 1059.900 \right]$
& $\left[ 441.371 \rightarrow 604.981 \right]$ \\ 
$m_{A_1}$ & $\left[ 638.813 \rightarrow 853.637 \right]$ & $\left[ 442.527
\rightarrow 640.705 \right]$ & $\left[ 670.550 \rightarrow 945.705 \right]$
& $\left[ 357.697 \rightarrow 516.760 \right]$ \\ 
$m_{A_2}$ & $\left[ 892.847 \rightarrow 1141.780 \right]$ & $\left[ 847.825
\rightarrow 1032.140 \right]$ & $\left[ 927.768 \rightarrow 1154.640 \right]$
& $\left[ 907.576 \rightarrow 1105.770 \right]$ \\ 
$m_{H^\pm}$ & $\left[ 783.823 \rightarrow 1111.600 \right]$ & $\left[
580.316 \rightarrow 779.945 \right]$ & $\left[ 842.585 \rightarrow 1143.880 %
\right]$ & $\left[ 856.237 \rightarrow 1007.360 \right]$ \\ \hline
$M_{44}^e$ & $\left[ 1327.510 \rightarrow 1622.510 \right]$ & $\left[
1219.930 \rightarrow 1491.020 \right]$ & $\left[ 1346.190 \rightarrow
1645.330 \right]$ & $\left[ 1029.900 \rightarrow 1247.770 \right]$ \\ 
$M_{55}^L$ & $\left[ 251.447 \rightarrow 307.323 \right]$ & $\left[ 200.000
\rightarrow 232.389 \right]$ & $\left[ 200.000 \rightarrow 225.176 \right]$
& $\left[ 290.963 \rightarrow 355.621 \right]$ \\ 
$\lvert \mu_{\func{sb}} \rvert$ & $\left[ 382.158 \rightarrow 467.079 \right]
$ & $\left[ 399.091 \rightarrow 487.777 \right]$ & $\left[ 432.895
\rightarrow 529.091 \right]$ & $\left[ 432.059 \rightarrow 528.067 \right]$
\\ \hline
$\Delta a_\mu \left[ 10^{-9} \right]$ & $\left[ 1.811 \rightarrow 3.410 %
\right] $ & $\left[ 1.810 \rightarrow 3.410 \right] $ & $\left[ 1.810
\rightarrow 3.410 \right] $ & $\left[ 1.810 \rightarrow 3.410 \right] $ \\ 
$\Delta a_e \left[ 10^{-13} \right]$ & $\left[ -6.730 \rightarrow -5.200 %
\right] $ & $\left[ -11.142 \rightarrow -5.985 \right] $ & $\left[ -7.207
\rightarrow -5.200 \right] $ & $\left[ -8.721 \rightarrow -5.200 \right] $
\\ 
$a_{hWW}$ & $\left[ 1.000 \rightarrow 1.000 \right] $ & $\left[ 1.000
\rightarrow 1.000 \right] $ & $\left[ 0.999 \rightarrow 1.000 \right] $ & $%
\left[ 1.000 \rightarrow 1.000 \right] $ \\ 
$R_{\gamma\gamma}$ & $\left[ 0.999 \rightarrow 0.999 \right] $ & $\left[
0.999 \rightarrow 0.999 \right] $ & $\left[ 0.999 \rightarrow 1.000 \right] $
& $\left[ 1.000 \rightarrow 1.000 \right] $ \\ \hline
$\chi^2$ & $\left[ 1.604 \rightarrow 2.750 \right]$ & $\left[ 1.501
\rightarrow 2.635 \right]$ & $\left[ 1.580 \rightarrow 2.761 \right]$ & $%
\left[ 1.509 \rightarrow 2.749 \right]$ \\ \hline
\end{tabular}
\captionof{table}{A scanned range of each parameter at case A, B, C and D.
$H_{1,2}$ mean non SM CP-even scalars and $A_{1,2}$ are non SM CP-odd scalars and $H^\pm$ stand for non SM charged scalars in this model. All data of $\Delta
a_{\mu,e}$ are collected within the $1\sigma$ constraint of each anomaly.} %
\label{tab:range_secondscan}}
\end{center}

\subsection{The muon and electron anomalous magnetic moments} \label{sec:second_paper_numeric_mueg2}

In order to confirm that our theoretical prediction for both anomalies can accommodate their constraints at $1\sigma$ and to analyze correlations between both anomalies and mass parameters, we take a case B in Table \ref{tab:parameter_region_best_peaked} since this benchmark point has the lowest value of the $\chi^2$ function when compared to other cases. The reason that the case B has the lowest value of the $\chi^2$ function arises from the obtained value of the electron anomaly, which is very close to the central experimental value. The four cases revealed the nearly central value of muon anomaly constraint at $1\sigma$, whereas the other cases except B revealed the nearly edge value of electron anomaly constraint at $1\sigma$. Therefore, the reason why the case B is most converged is related to whether our theoretical prediction for both anomalies can gain access to their central value of each anomaly constraint at $1\sigma$. For this reason, we take the case B in Table \ref{tab:range_secondscan} to study the correlations. The relevant parameter spaces are listed in Figure \ref{fig:relevant_parameters_delamue} and \ref{fig:relevant_parameters_vl_delamue}.

\begin{figure}[]
\centering
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.45]{DelaeDelamuMH1sb2.jpg} 
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.45]{DelaeDelamuMH2sb2.jpg} 
\end{subfigure} 
\par
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.45]{DelaeDelamuMA1sb2.jpg} 
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.45]{DelaeDelamuMA2sb2.jpg} 
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.45]{DelaeDelamuMHcsb2.jpg} 
\end{subfigure}
\caption{Available parameter spaces for the muon anomaly versus electron
anomaly with a mass parameter which attends the both anomalies$%
(H_{1,2},A_{1,2})$ and does not$(H^\pm)$. $H_{1,2}$ are non-SM CP even scalars, $%
A_{1,2}$ are non-SM CP odd scalars and $H^{\pm}$ are non-SM charged scalars.
All points in each plot are collected within $1\protect\sigma$ constraint of
each anomaly.}
\label{fig:relevant_parameters_delamue}
\end{figure}

\begin{figure}[]
\centering
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.50]{DelamuMe4Delaesb2.jpg} 
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.50]{DelaeDelamuMe4sb2.jpg} 
\end{subfigure} 
\par
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.50]{DelaeMe5Delamusb2.jpg} 
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[keepaspectratio,scale=0.50]{DelaeDelamuMe5sb2.jpg} 
\end{subfigure}
\caption{Available parameter spaces for the muon anomaly(electron anomaly)
versus a relevant vector-like mass $m_{e_4}(m_{e_5})$ with another
anomaly(two left plots) in bar where $m_{e_4}(m_{e_5})$ is simplified
notation for $M_{44}^{e}(M_{55}^{L})$, while the two right plots for the
muon anomaly versus electron anomaly with a vector-like mass $%
m_{e_4}(m_{e_5})$}
\label{fig:relevant_parameters_vl_delamue}
\end{figure}

To begin with, we consider the parameter spaces for the muon anomaly versus electron anomaly with a mass parameter which attends both anomalies $(H_{1,2}, A_{1,2})$ and does not $(H^\pm)$ in Figure \ref{fig:relevant_parameters_delamue}. Even thought the non-SM charged scalar does not attend both anomalies, the
similar pattern which the other scalars implement in Figure \ref%
{fig:relevant_parameters_delamue} is also appeared. We confirmed that mass of $H_2$ is nearly proportional to that of $H^\pm$, which causes the correlation identified in plots of the other non-SM scalars in Figure \ref{fig:relevant_parameters_delamue} is still maintained for the non-SM charged scalar. Interestingly, the case A, B and C in Table \ref{tab:range_secondscan} reported $m_{H_2}$ is nearly proportional to $m_{H^\pm}$ one-to-one ratio, whereas the case D revealed a fat proportion between them and still maintained the correlation.
\newline
As mentioned at the beginning of this section, we take the case B for the plots in Figure \ref{fig:relevant_parameters_delamue} and \ref{fig:relevant_parameters_vl_delamue} and a main distinction between the case B and others arises from the value of electron anomaly. If we take other cases instead of the case B to investigate the parameter spaces, the darker region appeared in top-left plot of Figure \ref{fig:relevant_parameters_delamue} will be shifted upward by locating at the value of $-5$ or $-6 \times 10^{-13}$ for the electron anomaly. In other words, the whole colored region in Figure \ref{fig:relevant_parameters_delamue} is shifted upwards to meet the scanned value of electron anomaly constraint at $1\sigma$, holding the correlations. Therefore, the white region appeared in Figure \ref{fig:relevant_parameters_delamue} is not strictly excluded region and affected by how well a benchmark point is converged and by a factor of $\kappa$. However, these plots still tells a correlation between both anomalies and a tendency that the lighter mass of $H_1$ is located at lower region of the parameter space. Mass of the lightest non-SM scalar $H_1$ implied in top-left plot of Figure \ref{fig:relevant_parameters_delamue} is ranged from $201$ to $246\func{GeV}$\cite{Hernandez-Sanchez:2020vax} and the cross section for this light non-SM scalar will be compared to that for SM Higgs in appendix. As for mass range of the other non-SM scalars confirmed in rest of other plots in Figure \ref{fig:relevant_parameters_delamue}, they all implied heavier mass than that of $H_1$ which can be flexible depending on how the parameters are converged as seen in each case of Table \ref{tab:range_secondscan}.
\newline~\newline
We investigate a correlation for an anomaly versus a relevant mass parameter with another anomaly in bar in Figure \ref{fig:relevant_parameters_vl_delamue}. Note that the fourth vector-like mass is relevant only for the muon anomaly, whereas the fifth is only for the electron anomaly. Even though the fourth(fifth) is irrelevant to the electron(muon) anomaly, it is good to express them together since we rearrange the mass parameter and the anomaly in bar for comparison. The top-left plot in Figure \ref{fig:relevant_parameters_vl_delamue} just fills in whole parameter region, thus no any correlation between the fourth vector-like mass and the muon anomaly is identified. After we rearranged the order of $m_{e_4}$ and $\Delta a_{\mu,e}$ from the top-left plot, we can confirm the similar correlation identified in Figure \ref{fig:relevant_parameters_delamue} from the top-right plot in Figure \ref{fig:relevant_parameters_vl_delamue}. The bottom-left plot identifies some correlation between the fifth vector-like mass and the electron anomaly contrary to the top-left plot. For the fifth vector-like mass, we put the constraint that the lightest vector-like mass should be greater than $200\func{GeV}$ \cite%
{Xu:2018pnq} and the mass region below $200\func{GeV}$ is all excluded. After rearranging the order of $m_{e_5}$ and $\Delta a_{\mu}$ as in the above plot, we confirmed the similar correlation appeared in the bottom-right plot. Interestingly, the top-right and the bottom-right plots checked the similar correlation.
\newline~\newline
We confirmed that the muon and electron anomalous magnetic moments with vector-like particles can be explained to within $1\sigma$ constraint of each anomaly in a unified way, which is based on two attributes; the first one is the extended scalar sector and the second one is related with the contributions of the vector-like leptons. The first one which is reflected in our prediction for both anomalies, consists of four non-SM scalars and these contributions play a crucial role for determining the magnitude of each anomaly. The second one is seen by two vertices of both anomaly diagrams. The other Yukawa interactions can take place at each vertex since the vector-like leptons come in the loop, which is differentiated by the case where the normal SM particles enter in the loop. To be more specific, the helicity flip mass caused by the vector-like fermions in the CP-even and CP-odd basis couples the initial particle inside the loop to another particle of different chirality, thus allowing different interactions at each vertex.  This means that the different sign problem can be solved by only considering multiplication of the Yukawa constants of each vertex and this property will be covered in detail in next subsection.

\subsubsection{How is the scalar exchange possible to accommodate both anomalies at $1\sigma$ constraint analytically?}

In order to %analysis 
analyze how the scalar exchange is able %possible 
to explain both anomalies within the $1\sigma$ range, 
%at $1\sigma$ constraint, 
we revisit the analytic expressions for both muon and electron anomalous
magnetic moments:
\begin{equation}
\begin{split}
\Delta a_{\mu }=y_{24}^{e}x_{42}^{e}\frac{m_{\mu }^{2}}{8\pi ^{2}}\Big[&
\left( R_{e}^{T}\right) _{22}\left( R_{e}^{T}\right) _{32}I_{S}^{(\mu
)}\left( m_{e_{4}},m_{H_{1}}\right) +\left( R_{e}^{T}\right) _{23}\left(
R_{e}^{T}\right) _{33}I_{S}^{(\mu )}\left( m_{e_{4}},m_{H_{2}}\right) \\
& -\left( R_{o}^{T}\right) _{22}\left( R_{o}^{T}\right) _{32}I_{P}^{(\mu
)}\left( m_{e_{4}},m_{A_{1}}\right) -\left( R_{o}^{T}\right) _{23}\left(
R_{o}^{T}\right) _{33}I_{P}^{\left( \mu \right) }\left(
m_{e_{4},}m_{A_{2}}\right) \Big], \\
\Delta a_{e}=y_{51}^{e}x_{15}^{L}\frac{m_{e}^{2}}{8\pi ^{2}}\Big[& \left(
R_{e}^{T}\right) _{22}\left( R_{e}^{T}\right) _{32}I_{S}^{(e)}\left(
m_{e_{5}},m_{H_{1}}\right) +\left( R_{e}^{T}\right) _{23}\left(
R_{e}^{T}\right) _{33}I_{S}^{(e)}\left( m_{e_{5}},m_{H_{2}}\right) \\
& -\left( R_{o}^{T}\right) _{22}\left( R_{o}^{T}\right)
_{32}I_{P}^{(e)}\left( m_{e_{5}},m_{A_{1}}\right) -\left( R_{o}^{T}\right)
_{23}\left( R_{e}^{T}\right) _{33}I_{P}^{\left( E\right) }\left(
m_{e_{5}},m_{A_{2}}\right) \Big],
\label{eqn:muon_electron_anomaly_prediction}
\end{split}%
\end{equation}
where
\begin{equation}
I_{S\left( P\right) }^{\left( e,\mu \right) }\left( m_{E_{4,5}},m_{S}\right)
=\int_{0}^{1}\frac{x^{2}\left( 1-x\pm \frac{m_{E_{4,5}}}{m_{e,\mu }}\right) }{%
m_{e,\mu }^{2}x^{2}+\left( m_{E_{4,5}}^{2}-m_{e,\mu }^{2}\right) x+m_{S,P}^{2}\left(
1-x\right) }dx  \label{eqn:loop_integrals}
\end{equation}
with $S(P)$ corresponding to scalar (pseudoscalar) and $E_{4,5}$ standing for the vector-like family. Furthermore, $E_{4}$ and $E_{5}$ only contribute to the muon and electron anomalous magnetic moments, respectively.

First of all, we focus on the sign %problem 
of each anomaly. The different signs of each anomaly indicated by the $%
1\sigma$ experimentally allowed range %constraint at $1\sigma$ 
can be understood at the level of Yukawa constants apart from the loop
structures. As seen in Table \ref{tab:parameter_region_initial_scan}, the
Yukawa coefficient $y$ can be either positive or negative, while $x$ only
remains positive since we take the absolute value to the $x$. 
%is taken to that. 
We also considered the case where the coefficients $x,y$ are purely
positive, assuming $v_3$ is positive, without taking absolute value and the
multiplication of the Yukawa coefficients $x \times y$ cannot change the
sign of each anomaly since the denominator of $x$ includes $y$ and they are
cancel out. Then, the sign problem depends on summing over loop functions and we found that the order of the muon anomaly prediction is
suitable, %while that of
whereas the corresponding to the electron anomaly is about $10^{-16}$ which
is too small to be accommodated within the %at $1\sigma$ constraint. 
$1\sigma$ experimentally allowed range. Therefore, we found that taking an
absolute value to one of the Yukawa coefficients is an appropriate strategy
for the sign and allows to reproduce the correct order of magnitude of each
anomaly %constraint at $1\sigma$.
allowed by the $1\sigma$ experimentally allowed range, for an appropiate
choice of the model parameters. This feature is a crucial difference compared with the $W$ or $Z^\prime$ gauge boson exchange\cite{CarcamoHernandez:2019ydc}. The $W$ gauge boson exchange covered in the main body of this work keeps the same coupling constant at each vertex, therefore it is completelly different from %exactly inconsistent with 
the scalar exchange with vector-like leptons. For the $Z^\prime$ exchange covered in \cite{CarcamoHernandez:2019ydc}, it has the common property that the coupling constant of each vertex is different to each other, whereas the coupling constants of the $Z^\prime$ are more constrained by the mixing angle between $i$th chiral family and fourth vector-like family, so it is impossible to explain both anomalies at the same time. As a result, allowing different Yukawa constants with appropiate signs enables both anomalies to be explained in a unified way. 
\newline
~\newline
Next we turn our attention to the order of magnitude of our predictions for both anomalies.
Considering that the sign problem is solved by having each Yukawa constant $%
y $ either positive or negative, it can be easily understood that inside
the structure in parentheses of Equation \ref%
{eqn:muon_electron_anomaly_prediction} should imply the same direction, which is 
%and the same direction 
is determined by the contribution of all loop functions in
parentheses. Since the mass difference among non-SM scalars and vector-like
particles is not so big, we have to consider their masses in the computation of muon and electron anomalous magnetic moments, as follows from Equation \ref%
{eqn:muon_electron_anomaly_prediction}. 
%we need to rely %depend 
%on delicate cancellation between the CP-even and CP-odd scalar contributions %on each loop functions 
%rather than considering some limiting cases based on very particular mass assumptions simplifying it by ignoring some mass scales. 
For an easy analysis, we take the case B reported in Table \ref%
{tab:parameter_region_best_peaked} and suppose that
\begin{equation}
\begin{split}
\left( R_e^T \right)_{22} \left( R_e^T \right)_{32} = c_1, \quad \left(
R_e^T \right)_{23} \left( R_e^T \right)_{33} = -c_1, \quad &\left( R_o^T
\right)_{22} \left( R_o^T \right)_{32} = c_2, \quad \left( R_o^T
\right)_{23} \left( R_o^T \right)_{33} = -c_2, \\
I_S^{\mu} \left( m_{e_4}, m_{H_1} \right) = d_1, \quad I_S^{\mu} \left(
m_{e_4}, m_{H_2} \right) = d_2, \quad &I_P^{\mu} \left( m_{e_4}, m_{A_1}
\right) = -d_3, \quad I_P^{\mu} \left( m_{e_4}, m_{A_2} \right) = -d_4, \\
I_S^{e} \left( m_{e_5}, m_{H_1} \right) = e_1, \quad I_S^{e} \left( m_{e_5},
m_{H_2} \right) = e_2, \quad &I_P^{e} \left( m_{e_5}, m_{A_1} \right) =
-e_3, \quad I_P^{e} \left( m_{e_5}, m_{A_2} \right) = -e_4, \\
d_1 > d_3 > d_2 > d_4, &\quad e_1 > e_3 > e_2 > e_4
\end{split}%
\end{equation}
where $c_{1,2}$ are arbitrary constant between $0$ and $1$ either positive
or negative and mass ordering among $d(e)_i, (i=1,2,3,4)$ can be easily
understood by considering mass difference between non-SM scalars and
vector-like particles. The muon and electron anomaly prediction can be
rewritten in terms of these redefined constants:
\begin{equation}
\begin{split}
\Delta a_\mu &= y_2 x_2 \frac{m_\mu^2}{8\pi^2} \left[ c_1 d_1 - c_1 d_2 + c_2
d_3 - c_2 d_4 \right] \\
&= y_2 x_2 \frac{m_\mu^2}{8\pi^2} \left[ c_1 \left( d_1
- d_2 \right) + c_2 \left( d_3 - d_4 \right) \right] = y_2 x_2 \frac{m_\mu^2%
}{8\pi^2} \left[ c_1 d_{12} + c_2 d_{34} \right] \\
\Delta a_e &= y_1 x_1 \frac{m_e^2}{8\pi^2} \left[ c_1 e_1 - c_1 e_2 + c_2 e_3
- c_2 e_4 \right] \\
&= y_1 x_1 \frac{m_e^2}{8\pi^2} \left[ c_1 \left( e_1 - e_2
\right) + c_2 \left( e_3 - e_4 \right) \right] = y_1 x_1 \frac{m_e^2}{8\pi^2}
\left[ c_1 e_{12} + c_2 e_{34} \right]
\end{split}%
\end{equation}
where $y_2,x_2,y_1,x_1$ are simplified notation for $%
y_{24}^e,x_{42}^e,y_{51}^e,x_{15}^L$, respectively, and $d(e)_{ij} \equiv
d(e)_i - d(e)_j$ and $d(e)_{ij}$ are positive. Since the inside structure in
parentheses depends on relative magnitude of both $c_{1,2}$ and $d(e)_{ij}$
at this stage where no more analytic simplication is possible, it is good to
implement a specific value for them. Referring the values used to derive the
result of case B, they are
\begin{equation}
\begin{split}
y_2 x_2 \frac{m_\mu^2}{8 \pi^2} c_1 d_1 = 1.494 \times 10^{-7}, &\quad y_1
x_1 \frac{m_e^2}{8 \pi^2} c_1 e_1 = -2.237 \times 10^{-12} \\
-y_2 x_2 \frac{m_\mu^2}{8 \pi^2} c_1 d_2 = -1.338 \times 10^{-7}, &\quad
-y_1 x_1 \frac{m_e^2}{8 \pi^2} c_1 e_e = 1.028 \times 10^{-12} \\
y_2 x_2 \frac{m_\mu^2}{8 \pi^2} c_2 d_3 = -9.839 \times 10^{-8}, &\quad y_1
x_1 \frac{m_e^2}{8 \pi^2} c_2 e_3 = 8.406 \times 10^{-13} \\
-y_2 x_2 \frac{m_\mu^2}{8 \pi^2} c_2 d_4 = 8.541 \times 10^{-8}, &\quad -y_1
x_1 \frac{m_e^2}{8 \pi^2} c_2 e_4 = -4.631 \times 10^{-13}
\label{eqn:middle_values_for_prediction}
\end{split}%
\end{equation}
and summing over all values in left or right column of Equation \ref%
{eqn:middle_values_for_prediction} yields the prediction for muon and
electron anomaly at $1\sigma$
\begin{equation}
\begin{split}
\Delta a_\mu &= y_2 x_2 \frac{m_\mu^2}{8\pi^2} \left[ c_1 d_1 - c_1 d_2 +
c_2 d_3 - c_2 d_4 \right] = 2.688 \times 10^{-9} \\
\Delta a_e &= y_1 x_1 \frac{m_e^2}{8\pi^2} \left[ c_1 e_1 - c_1 e_2 + c_2
e_3 - c_2 e_4 \right] = -8.310 \times 10^{-13}.
\end{split}%
\end{equation}

\section{Conclusion} \label{sec:second_paper_conclusion}

We have proposed a model to account for the hierarchical structure of the SM Yukawa couplings.
%constants in SM and 
In our approach 
%and by the assumption that %belief 
%that 
the SM is an effective theory arising from a theory with extended particle
spectrum and symmetries.
% aftye the spontaneously broken from higher energy scale as low as $\func{TeV}$, 
The considered model includes 
%the BSM model that is extended by the global $U(1)^\prime$ symmetry and features both a 2HDM and a Fermiophobic $Z^\prime$ model with two vector-like families as well as a flavon.
an extension of the 2HDM where the particle spectrum is enlarged by the
inclusion of two vector-like fermion families, right handed Majorana neutrinos and a
gauge singlet scalar field, together with 
the inclusion of a global $U(1)^\prime$ symmetry spontaneously broken at the 
$\func{TeV}$ scale. %which acquires  and gauge symmetry is 
Since the $U(1)^\prime$ symmetry is global, this model does not feature 
a $Z^\prime$ boson and it is softly broken in the 2HDM potential to avoid a Goldstone boson. 
Its main effect is to forbid SM Yukawa interactions due
to the $U(1)^\prime$ charge conservation. 
%quantum numbers. 
Besides that, this model has the
property of the 2HDM type II where one Higgs doublet couples with the up-type fermions whereas the remaining one has Yukawa interactions with down-type fermions, where such couplings are allowed between chiral fermions and vector-like fermions due to the choice of 
$U(1)^\prime$ charges (chiral fermions having zero charges while vector-like fermions, Higgs and flavons have charges $\pm 1$).
%up-type fermions are governed by up-type SM Higgs while down-type fermions are suitable for down-type SM Higgs. 
Below the mass scale of the vector-like fermions, such couplings result in effective Yukawa couplings suppressed by a factor 
$\left\langle \phi \right\rangle/M$ where the numerator is the vev of the flavon
and the denominator is the vector-like mass. This factor naturally determines
the magnitude of SM interactions and the mass scale for the vector-like
fermions under a suitable choice of the flavon vev. 
We have developed a mixing formalism based on $7 \times 7$ mass matrices to describe the mixing 
of the three chiral families with the two vector-like
families. 
\newline~\newline
Within the above proposed model, 
we have focused on accommodating the long-established muon and less established electron anomalous
magnetic moments at one-loop level. A main difficulty arises from the sign of each anomalous deviation of the experimental value from its SM prediction. Generally, the Feynman diagrams for the muon
and electron anomalous magnetic moments have the same structure except from the fact that the external particles are different, which makes it difficult to flip the sign of each contribution. Specifically we have required that both deviations in 
Equation \ref{eqn:deltaamu_deltaae_at_1sigma}) 
at one-loop should be accommodated within the $1\sigma$ experimentally allowed range,
which is a challenging requirement. %
\newline
~\newline
%Once the flavon develops its vev and mixing between SM and heavy fermions
%scalars 
%takes place, the mass matrices are diagonalized by a mechanism so
%called ``universal seesaw", \Antonio{where the heavy mass scale of the vector like fermions plays a crucial role in explaining the SM charged fermion mass hiearchy.}%due to involving a few of different mass scales.
%These diagonalized mass matrices can be written in two basis, one of which
%is called the convenient basis and the other \Antonio{one} is the decoupling basis. 
%Since we are interested in explaining both anomalies, the lepton sector is treated in main body and the quark sector is covered in appendix. \newline
%~\newline
We first considered in detail the $W$ boson exchange contributions to the muon and electron 
anomalous magnetic moments at one-loop.
The relevant sector for the $W$ boson exchange is that of the neutrino and we analyzed a novel
operator that generates the masses of the light active neutrinos in this model. 
The well-known five dimensional Weinberg
operator which we refer as type Ia seesaw mechanism does not work in this model 
since it is forbiden by the $U(1)$ symmetry due to the fact that both $SU(2)$ scalar doublets are negatively charged under this symmetry. 
%charged since it is they are very subleading and thus will give a tiny contribution to the light active neutrino masses.
%since the SM Higgses are negatively charged under the extended gauge symmetry. 
For this reason, we made use of the Weinberg-like operator known as
type Ib seesaw mechanism allowed in this model. With the type Ib seesaw
mechanism, we built the neutrino mass matrix with two vector-like neutrinos and ignored fifth vector-like neutrinos since they are too heavy to
contribute to the phenomenology. The deviation of unitarity $\eta$ derived
from the heavy vector-like neutrinos plays a crucial role for enhancing the
sensitivity of the CLFV $\mu \rightarrow e \gamma$ decay to the observable
level. Furthermore, the Yukawa constants of Dirac neutrino mass matrix can be connected to the observables measured in neutrino oscillation experiments. %Another interesting feature of the model is the fact that the Yukawa constants of Dirac neutrino mass matrix can be connected to the observables measured in neutrino oscillation experiments . 
One of the neutrino Yukawa constants is defined with a
suppression factor $\epsilon$. Therefore, the effective $3 \times 3$
neutrino mass matrix tells that the tiny masses of the light active neutrinos depend on the mass scale of vector-like neutrinos as well as on the suppression factor $\epsilon$. %
%on not only mass of vector-like neutrinos but also the suppression factor $\epsilon$. 
This implies that mass scale of vector-like neutrinos is not required to be of the order 
% does not need to be is not necessarily be order 
of $10^{14}$ GeV, as in %which is required for 
the conventional type Ia seesaw mechanism. 
In our proposed model, the vector-like neutrinos can have masses at the $\func{TeV}$ scale, thus allowing to test our model at colliders. Those vector-like neutrinos can be pair produced at the LHC via Drell-Yan annihilation mediated by a virtual $Z$ gauge boson. They can also be produced in association with a SM charged lepton via Drell-Yan annihilation mediated by a $W$ gauge boson. These heavy vector like sterile neutrinos can decay into a SM charged lepton and light active neutrinos. Thus, the heavy neutrino pair production at a proton-proton collider will give rise to an opposite sign dilepton final state, which implies that the observation of an excess of events in this final state over the SM background can be a smoking gun signature
of this model, whose observation will be crucial to assess its viability. 
%we can expect order of vector-like neutrinos to be $\func{TeV}$ scale and might confirm presence of those in close future experiments. \newline
%~\newline
It is confirmed that the branching ratio of $\mu \rightarrow e \gamma$ decay
can be expressed in terms of the deviation of unitarity $\eta$ as shown in %from the
%references
\cite{Hernandez-Garcia:2019uof,Calibbi:2017uvl} and our prediction
for the muon and electron anomalous magnetic moments can also be written in
terms of non-unitarity. We derived the analytic expression for the anomalies
and found that the order of magnitude of these predictions is too small to accommodate the
experimental bound within the $1\sigma$ range and the sign of each prediction also points
out in the same direction. Therefore, we concluded that the $W$ boson exchange at
one-loop is not enough to explain both anomalies at $1\sigma$ and this
conclusion has been a good motivation to search for another possibility such
as scalar exchange, which is one of the main purposes of this work.  
\newline
~\newline
We then turned our attention to the 2HDM contributions (inclusion also of the singlet scalar $\phi$) to the muon and electron 
anomalous magnetic moments, assuming by a choice of parameters a diagonal charged lepton mass matrix to 
suppress the branching ratio of $\mu \rightarrow e \gamma$. In our analysis
we considered in detail the scalar sector of our model, which is composed of 
%features 
%three scalars,} 
%two of them SM Higgses $H_{u,d}$ and the rest is flavon $\phi$, a
two $SU(2)$ scalar doublets $H_u$ and $H_d$ and one electrically neutral complex scalar $\phi$ by studying the corresponding scalar potential, deriving the squared mass matrices for the CP-even, CP-odd neutral and electrically charged scalars and determining the resulting scalar mass spectrum.
% scalar potential consisting of the scalars can be constructed, and then the mass matrix for
% CP-even, CP-odd neutral and charged scalars are discussed in the basis of
% real and imaginary part of each scalar. 
We have restricted to the scenario corresponding to the decoupling limit where %Here, we assume that 
no mixing between the physical SM Higgs $h$ and the physical non-SM scalars $H_{1,2}$
arise and within this scenario we have imposed the restrictions arising from %cover 
the Higgs diphoton decay rate, the $hWW$ coupling, the $125$ GeV mass of the SM-like Higgs and the experimental lower bounds on non SM scalar masses, to determine the allowed parameter space consistent with the muon and electron anomalous magnetic moments. To this end, we have constructed a $\chi^2$ fitting function, which measures the deviation of the values of the physical observables obtained in the model, i.e., $(g-2)_{e,\mu}$, the $125$ GeV SM-like Higgs mass, the Higgs diphoton signal strength, the $hWW$ coupling, with respect to their experimental values. Its minimization allows to determine the values of the model parameters consistent with the measured experimental values of these observables. 
%required to setup the fitting function $\chi^2$. 
After saturating the $\chi^2$ value less than or nearly
2, we obtained four independent benchmark points and carried out second scan with
the benchmark points to find a correlation between observables and mass
parameters. For the plots, we took a case most converged when compared to other
ones. We found that our prediction for both anomalies can be explained
within the $1\sigma$ constraint of each anomaly and a correlation inversely
proportional for muon versus electron anomaly is appeared in Figure \ref%
{fig:relevant_parameters_delamue} and \ref%
{fig:relevant_parameters_vl_delamue}. Here, we put two constraints on mass
of the lightest non-SM scalar and of the lightest vector-like family; $%
m_{H_1}, m_{e_5} > 200\func{GeV}$ based on references. The second scan result tells that the available parameter space is not significantly constrained by current experimental
results on non-SM scalar mass and vector-like mass, while keeping
perturbativity for quartic couplings and Yukawa constants. Lastly, we
discussed how we were able to explain both $(g-2)_{e,\mu}$ anomalies at $1\sigma$ constraint
and impact of the light non-SM scalar $H_1$. For the former, we first
simplified the prediction for both anomalies and used some numerical values at
the stage where no more analytic simplication is possible. For the latter,
we compared the cross section for the SM process $pp \rightarrow h$ and BSM process $pp \rightarrow H_1$ and included this comparison in Appendix~\ref{B}. 

We conclude that the proposed model of fermion mass hierarchies 
is able to successfully accommodate both the muon and electron anomalous magnetic moments within the $1\sigma$ experimentally allowed ranges, with the dominant contributions arising from one loop diagrams involving the 2HDM scalars and vector-like leptons.
The resulting model parameter space consistent with the $(g-2)_{e,\mu}$ anomalies requires masses of non-SM scalars and vector-like particles in the sub TeV and TeV ranges, thus making these particles accessible at the LHC and future colliders.
   %   prediction for both anomalies at one-loop level can
% accommodate each constraint at $1\sigma$ and predicted non-SM scalars and
% vector-like particles could be revealed by the forthcoming experiments.
